An unfitted radial basis function generated finite difference method applied to thoracic diaphragm simulations

The thoracic diaphragm is the muscle that drives the respiratory cycle of a human being. Using a system of partial differential equations (PDEs) that models linear elasticity we compute displacements and stresses in a two-dimensional cross section of the diaphragm in its contracted state. The boundary data consists of a mix of displacement and traction conditions. If these are imposed as they are, and the conditions are not compatible, this leads to reduced smoothness of the solution. Therefore, the boundary data is first smoothed using the least-squares radial basis function generated finite difference (RBF-FD) framework. Then the boundary conditions are reformulated as a Robin boundary condition with smooth coefficients. The same framework is also used to approximate the boundary curve of the diaphragm cross section based on data obtained from a slice of a computed tomography (CT) scan. To solve the PDE we employ the unfitted least-squares RBF-FD method. This makes it easier to handle the geometry of the diaphragm, which is thin and non-convex. We show numerically that our solution converges with high-order towards a finite element solution evaluated on a fine grid. Through this simplified numerical model we also gain an insight into the challenges associated with the diaphragm geometry and the boundary conditions before approaching a more complex three-dimensional model.

==> sections/10_experiments_benchmark_Robin.tex <==
\section{\victor{Benchmark II: Deformation of the diaphragm using the smoothed Robin boundary conditions}}
\label{sec:experiments:Robin}
This benchmark includes a more difficult problem compared with Benchmark I from Section 
\ref{sec:experiments:dirichlet}. As discussed in Section \ref{section:diabehavior}, we can measure 
the displacements over certain parts of the boundary, i.e., where the diaphragm is fixed near the spine, or where it moves together 
with the sternum and some ribs. In the regions where the displacements are not known, 
we may instead have information about the thoracic or abdominal pressure. A pressure condition is a special case of a traction boundary condition. 
A straightforward way to handle these boundary conditions would be to impose the Dirichlet condition (the known displacements) 
and the traction condition (the known traction values) in disjoint regions. This implies a discontinuous imposition of boundary conditions, 
for which: (i) we can not obtain high-order convergence according to our preliminary tests, (ii) 
the resulting deformation might be discontinuous or have large local derivatives, which would not reflect 
the physicological behavior of the diaphragm. For this reason we introduce a smooth blending of the Dirichlet and the traction 
boundary conditions in Robin form~\eqref{eq:model:secondNewton_bcs_Robin}.

This setting implies that we solve the system of equations \eqref{eq:method:DandF},
where the supports of the Robin coefficients $\kappa_0(y)$ and $\kappa_1(y)$ are chosen to overlap slightly in the regions where the type of boundary data changes.
In Figure \ref{fig:experiments:Diaphragm:Robin:coefficients} we display the Robin coefficients which we use in Benchmark II. 
The displayed coefficients are a function of the boundary parameter $t$. 
The coefficients were computed using a sum of the sigmoid functions $\frac{1}{1+e^{\varepsilon (t-d_i)}}$, where $\varepsilon = \pm 20$, 
$t$ is the boundary parameter and $d_i$, $i=1,2,..$ are the transition points 
(marked by dashed lines in Figure \ref{fig:experiments:Diaphragm:Robin:coefficients}). The 
sign of $\varepsilon$ depends on whether the coefficient is increasing (positive sign) or decreasing (negative sign).

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.65\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Data/bndry_coefficients.pdf}

    \caption{The Robin boundary coefficients displayed over the diaphragm show the impositions of the traction 
    and the Dirichlet parts of the boundary condition. The orange line corresponds to the traction coefficient $\kappa_1$, 
    and the blue line corresponds to the Dirichlet coefficient $\kappa_0$. The dashed lines show the location of the end 
    points of the diaphragm (regions 2 and 8 in Figure~\ref{fig:smoothing:bcPosition}). The parameter $t$ corresponding 
    to the boundary of the diaphragm is illustrated in Figure \ref{fig:boundary}.}

    \label{fig:experiments:Diaphragm:Robin:coefficients}
\end{figure}
The smoothed boundary displacement values $g_1$, $g_2$ and the boundary traction values $h_1$, $h_2$ are given in Figure \ref{fig:experiments:Diaphragm:Robin:boundary_data}. 
Through the functions $g_1$ and $g_2$ we impose thickening in the regions 2, 3, 7 and 8 based on the distribution in Figure \ref{fig:smoothing:bcPosition}. 
Additionally, we also impose a gentle translation in the negative vertical direction in the regions 7 and 8. 
Through the functions $h_1$ and $h_2$ we impose the translation of zone 5 in the negative vertical direction.
\begin{figure}[h!]
    \centering
    \begin{tabular}{@{}c@{}cc@{}}
      %\multicolumn{2}{c}{\textbf{Displacements }$\mathbf{\tilde u_1}$} \\
      &\hspace*{8mm}\textbf{Dirichlet data} & \hspace*{4mm}\textbf{Traction data} \\
      \rotatebox{90}{\hspace*{4mm}\textbf{Displacements }$\mathbf{\tilde u_1}$}  
        &\includegraphics[width=0.48\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Data/u1_Dirichlet_smooth.pdf} & 
        \raisebox{0.005\linewidth}{\includegraphics[width=0.445\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Data/u1_Traction_smooth.pdf}} \\
        %\multicolumn{2}{c}{\textbf{Displacements }$\mathbf{\tilde u_2}$} \\
        \rotatebox{90}{\hspace*{4mm}\textbf{Displacements }$\mathbf{\tilde u_2}$}
        &\hspace{0.04\linewidth}\includegraphics[width=0.45\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Data/u2_Dirichlet_smooth.pdf} &
        \raisebox{0.01\linewidth}{\includegraphics[width=0.465\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Data/u2_Traction_smooth.pdf}}
    \end{tabular}
    \caption{Benchmark II: The smoothed boundary data over the diaphragm. For this benchmark we have both Dirichlet data (left column) 
    and traction data (right column), each with a horizontal component (first row) and a vertical component (second row). 
    The markers show the initially placed data points, which are then linearly interpolated into $\tilde{M}_g=80$ data points. 
    For the approximation, $N_g=120$ node points and stencil size $n=28$ were used. 
    \victor{The dashed lines show the location of the end points of the diaphragm (regions 2 and 8 in Figure~\ref{fig:smoothing:bcPosition}). 
    The parameter $t$ corresponding to the boundary of the diaphragm 
    is illustrated in Figure \ref{fig:boundary} (right image).}}
    \label{fig:experiments:Diaphragm:Robin:boundary_data}
\end{figure}
\subsection{Solution of Benchmark II}
The solution is given in Figure \ref{fig:experiments:Diaphragm:Robin:solution}, where we can see the spatial distribution of 
displacements and the Von Mises stress. To obtain this figure we used $h=0.006$, $p=5$, and $q=5$. We observe that 
there is a slight thickening in regions 2, 3, 7 and 8, according to the labels from Figure \ref{fig:smoothing:bcPosition}, which 
corresponds to the imposed thickening up to some extent. In regions 4 and 6, we observe a slight bend towards the interior, and in 
region 5, a translation in the negative vertical direction. This behavior does not entirely mimic the physiological contraction of 
the diaphragm, 
however, constructing a more accurate model is planned as future work. 
This solution serves as a test to understand whether the
unfitted RBF-FD method can handle the problem with the smoothed Robin boundary condition, 
as well as to explore how this type of boundary condition affects the behaviour of the solution. 
%\begin{figure}[h!]
%    \centering
    
%    \begin{tabular}{c}
%    \textbf{Displacement $\mathbf{\tilde u_1}$} \\
%    \includegraphics[width=0.85\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Solution/solution_numRef_abs_u1.png} \\
%    \textbf{Displacement $\mathbf{\tilde u_2}$} \\
%    \includegraphics[width=0.85\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Solution/solution_numRef_abs_u2.png} \\
%    \textbf{Von Mises stress} \\
%    \includegraphics[width=0.85\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Solution/solution_numRef_abs_vonMises.png}
%    \end{tabular}
%    \caption{Benchmark II: This solution was obtained using the unfitted RBF-FD discretization with internodal distance $h=0.002$, 
%    an oversampling parameter $q=5$ and an appended polynomial basis of degree $5$. 
%    \victor{The conventional displacement and stress units are normalized using the scaling $s_{\Omega} = 0.15692^{-1}\, \text{m}^{-1} = 156.92^{-1}\, \text{mm}^{-1}$, provided in Section \ref{sec:smooth}.}}
%    \label{fig:experiments:Diaphragm:Robin:solution}
%\end{figure}
\begin{figure}[h!]
    \centering
    
    \begin{tabular}{c}
    \textbf{Displacement $\mathbf{\tilde u_1}$} \\
    \includegraphics[width=0.65\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Solution/solution_numRef_abs_u1.png} \\
    \textbf{Displacement $\mathbf{\tilde u_2}$} \\
    \includegraphics[width=0.65\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Solution/solution_numRef_abs_u2.png} \\
    \textbf{Von Mises stress} \\
    \includegraphics[width=0.65\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Solution/solution_numRef_abs_vonMises.png}
    \end{tabular}
    \caption{Benchmark II: The computed displacements and the corresponding von Mises stress over the diaphragm. 
    This solution was obtained using the unfitted RBF-FD discretization with internodal distance $0.006$, an oversampling parameter 
    $q=5$ and an appended polynomial basis of degree $p=5$. \victor{Due to the scaling applied to the geometry (see Section~\ref{sec:smooth}), 
    the displayed results for displacement and stress should be multiplied with $s_{\Omega}^{-1}=0.15692$ m to recover the results corresponding 
    to the unscaled problem.}}
    \label{fig:experiments:Diaphragm:Robin:solution}
\end{figure}


\subsection{Convergence under node refinement}
We validate the numerical solution by studying convergence under node refinement. 
Our choice of reference solution for this study is a fine solution computed using the unfitted RBF-FD method with an internodal distance 
$h=0.002$ and a polynomial degree $p=5$ used for constructing the local approximations. 
The relative error against the reference solution is computed using~\eqref{eq:dirichlet:error}. 
The relation between the considered $h$ and the number of points $N$ in $X$ is given in Table~\ref{fig:experiments:Dirichlet:Diaphragm:h_to_N_table}.

The errors for different choices of the polynomial degree $p$ are displayed in Figure \ref{fig:experiments:Diaphragm:Robin:convergence_selfRef}. 
\elisabeth{We do not observe convergence for any $p$ when $h$ is too large.} The reason for this is that the problem is not resolved yet. 
When $h$ is sufficiently small, and when $p=4$ or $p=5$, the solution converges at least with order $p-1$, which is desired. When $p=2$, 
we do not see convergence, since we would need an even higher resolution for this (small) polynomial degree. When $p=3$ we observe an approximately 
first order convergence for a sufficiently small $h$. This order is expected to increase to $p-1=2$ if $h$ is refined further. Low-order or no convergence 
when $p$ is small advocates using a higher order method.

\begin{figure}[h!]
    \centering
    \begin{tabular}{ccc}
        \hspace{0.8cm}\textbf{Displacement }$\mathbf{\tilde u_1}$ & \hspace{0.8cm}\textbf{Displacement }$\mathbf{\tilde u_2}$ & \hspace{0.8cm}\textbf{Von Mises} \\
        \includegraphics[width=0.3\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Convergence/Self/Error_u1.pdf} &  
        \includegraphics[width=0.3\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Convergence/Self/Error_u2.pdf} &  
        \includegraphics[width=0.3\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Convergence/Self/Error_stress.pdf}  
    \end{tabular}
    % \begin{tabular}{cc}
    % \hspace{1cm}$p=2$ & \hspace{1cm}$p=3$ \\
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Convergence/Self/Error_polydeg=2.pdf}  &  
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Convergence/Self/Error_polydeg=3.pdf} \\
    % \hspace{1cm}$p=4$ & \hspace{1cm}$p=5$ \\
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Convergence/Self/Error_polydeg=4.pdf}  &  
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Convergence/Self/Error_polydeg=5.pdf}
    % \end{tabular}
    \caption{Benchmark II: Convergence of the displacements $\tilde u_1$ and $\tilde u_2$ and the Von Mises stress for different polynomial degrees $p$, 
    towards a dense numerical reference computed using the unfitted RBF-FD-LS method with $h=0.002$, $p=5$.}
    \label{fig:experiments:Diaphragm:Robin:convergence_selfRef}
\end{figure}

The spatial distribution of the error computed using $h=0.006$ and $p=5$ is given in Figure
\ref{fig:experiments:Diaphragm:Robin:error_spatial_selfRef}. Here the error is largest close to 
region 5 from Figure \ref{fig:smoothing:bcPosition}, where we have enforced the traction boundary 
condition, which includes derivatives. In our experience the error is normally larger in the regions 
where derivative boundary conditions are imposed compared with the regions where a Dirichlet condition is 
imposed, and we also observed this in \cite{tominec2020unfitted,ToLaHe20}.
\begin{figure}[h!]
    \centering
    
    \begin{tabular}{cc}
    \textbf{Displacement $\mathbf{\tilde u_1}$} & \textbf{Displacement $\mathbf{\tilde u_2}$} \\
    \includegraphics[width=0.49\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Error_distribution/err_numRef_abs_u1.png} &
    \includegraphics[width=0.49\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Error_distribution/err_numRef_abs_u2.png} \\
    \multicolumn{2}{c}{\textbf{Von Mises stress}} \\
    \multicolumn{2}{c}{\includegraphics[width=0.6\linewidth]{pics/experiments_highorder_customData/Diaphragm/Robin/Error_distribution/err_numRef_abs_vonMises.png}}
    \end{tabular}
\caption{Benchmark II: Error distribution in logarithmic scale for $h=0.006$ and $p=5$ when a fine unfitted RBF-FD-LS solution ($h=0.002$, $p=5$) 
         is taken as reference for computing the error.}
    \label{fig:experiments:Diaphragm:Robin:error_spatial_selfRef}
\end{figure}


==> sections/11_conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

The unfitted RBF-FD method in the least-squares setting \cite{tominec2020unfitted} provided a robust framework 
for solving the linear elasticity system of PDEs over the simplified diaphragm geometry. 

We could also use the unfitted RBF-FD method to smooth the geometry curve and the boundary data. 
Ensuring that all components of the model were smooth allowed us to achieve high-order convergence, which reduces the number of unknowns 
needed for a given approximation error. In the experiments (not unexpectedly), Benchmark II, with Robin boundary conditions, proved more 
challenging to solve than Benchmark I with Dirichlet conditions. We needed higher resolution to achieve the same error level, and we did 
not see any convergence for the larger values of $h$. In the error plots, we could also see that the error is largest in the area where only 
the traction condition is active.
% An unfitted RBF-FD method allowed  to use when solving PDEs on a high-aspect ratio geometry such as the diaphragm. 
% Consider the node layout in Figure~\ref{fig:method:diaphragm_interpNodes}. 
% If we were using a body-fitted node set with the same spatial resolution, we would have approximately one node point in the thickness direction. 
% The stencil shape acquired around any interior point would in this case be highly skewed, not only on the boundary, but also in all interior points. 
% Skewed stencils lead to a worse approximation error compared to when using a perfectly round stencil \cite{tominec2020unfitted}.
% 
% We observed a benefit of the unfitted RBF-FD method with respect to the high-aspect ratio geometry. 
% Consider the node layout in Figure~\ref{fig:method:diaphragm_interpNodes}. 
% If we were using a body-fitted node set with the same spatial resolution, we would have approximately one node point 
% in the thickness direction. This would not be enough to resolve the problem and hence, we would need a higher resolution, 
% leading to a higher computational cost. 
% 
% 
%In Benchmark II it was hard to manually choose the boundary data to properly mimic the physiological behavior of the diaphragm. 
%\elisabeth{It is very important to perform the simulations using the real Dirichlet and traction data, which we are planning to use in the future.}
In the present work, we manufactured the data for the boundary conditions, but the aim is to eventually use measured pressure values 
and the solid body rotation of the ribs as boundary input data. This is most similar to the more challenging Benchmark II. 
There are a large number of transition zones, where the type of boundary condition changes, while we still expect a smooth 
behaviour of the solution. We were able to achieve a smooth solution and high-order convergence by using the proposed smoothing approach, 
and we will use that for the real application. Further investigations are needed regarding how to choose smoothing parameters such as the size of the transition zone.

To validate the unfitted RBF-FD solver, we measured convergence both against a self reference and against a highly resolved linear FEM solution. 
The results show that the two methods agree to high accuracy. 

Future work includes employing an unfitted RBF-FD-LS method to solve a more complex elastic problem, 
where we are going to use the 3D geometry and forcing data, both extracted from the CT (computed tomography) images of the diaphragm.

%An advantage of the RBF-FD method is that the solution can be represented with 
%significantly fewer unknowns. It is also easy to implement the Robin boundary conditions.

% old
% The unfitted RBF-FD method in the least-squares setting \cite{tominec2020unfitted} provided an accurate and a robust framework for smoothing the geometry data, boundary data, 
% and for computing solutions to a system of PDEs (linear elasticity) over the simplified diaphragm geometry. This is a ground result that we need in order to tackle 
% a more realistic diaphragm problem in the future.

% A basic finite element solver gives an answer close to the answer of our solver, as can be observed from the convergence test in Benchmark I (Section \ref{sec:experiments:dirichlet}), 
% where we measure the convergence of our solution to a finite element reference solution. 

% In Benchmark II (Section \ref{sec:experiments:Robin}), smoothed Robin-type boundary conditions \eqref{eq:model:secondNewton_bcs_Robin} allowed for a smooth solution and high-order convergence. 
% We will use this concept for more complex modeling.

% The error in Benchmark I is significantly smaller compared with the error in Benchmark II. We also need a larger amount of 
% degrees of freedom in Benchmark II, so that the solution started converging at all.

% In Benchmark II it was hard to manually choose the boundary data to properly mimic the physiological behavior of the diaphragm. 
% \elisabeth{It is very important to perform the simulations using the real Dirichlet and traction data, which we are planning to use in the future. }

% Our computations are based on the isotropic placement of interpolation points. None of the spatial error 
% distribution tests that we performed is indicating that the error is significantly larger in the 
% thickness direction of the diaphragm. Instead, the error is larger in magnitude when the shape of the diaphragm is locally concave (Benchmark I), 
% where the Von Misses stress is large (Benchmark I), or close to the regions where the Traction condition is imposed (Benchmark II). 
% In this sense we believe that \elisabeth{in our case} a pre-set 
% anisotropic node placement in the 
% thickness direction is not needed. In turn, we believe that an adaptive node refinement governed by a 
% good choice of an error indicator is a more general approach which would help 
% in reducing the error.

==> sections/12_acknowledgements.tex <==
\section*{Acknowledgments}
The INVIVE project is funded by the Swedish Research Council, grant number 2016-04849.

==> sections/1_introduction.tex <==
\section{Introduction}
% WHY is it important to study the diaphragm
During the 2020 covid-19 pandemic we have all been made aware that intensive care units (ICU) have limited capacity with respect to the number of patients that can be cared for at the same time. The WHO report on covid-19 in China~\cite{WHO} indicates that covid-19 patients with severe symptoms need 3--6 weeks in ICU.
Patients with severe respiratory symptoms are put under mechanical ventilation to save their lives. At the same time, the mechanical ventilation has adverse effects, such as ventilator induced diaphragmatic dysfunction (VIDD)~\cite{Cacciani}, which prolongs the ICU time.  Hence, improving mechanical ventilation can have a significant impact on ICU patient turnover. 

This work is part of the INVIVE project\footnote{\url{https://www.it.uu.se/research/scientific_computing/project/rbf/biomech}}, 
where we aim to create a mechanically ventilated virtual patient~\cite{KZECH15}
on whom we can perform tests with different ventilation strategies and counter measures against VIDD~\cite{Jaber17}. With the virtual patient, we can also vary the gender, physiology, age and potential injuries that affect the response. Using simulations allows to create a controlled computer-based environment in a way that is not possible in a clinical setting.
%Proper simulation tools also reduce the need for animal experiments in research. Finally, virtual patients are central in ICU training~\cite{icutraining}, but the diaphragm is still missing in simulators.


% The diaphragm is the most important muscle.
The diaphragm is the main respiratory muscle, and the present focus of our study. The diaphragm is located between the thoracic and abdominal cavities. It has two domes, and is attached to the lower ribs, the spine, and the sternum. 
During mechanical ventilation, the normal action of the diaphragm, where inhalation follows the contraction of the muscle, is reversed, i.e., 
the muscles become passive and the air is pumped into the lungs by the ventilator. As air is entering the lungs with a positive pressure, the muscle fibres 
are instead extended. This sudden and extreme mechanical perturbation is the trigger of a chain of biological events causing 
the progression of VIDD.

%--------------------------------------------------------------------------

% WHICH are the numerical challenges. This maybe includes the surrounding muscles and attachments. 
% anisotropy boundary conditions non-linearity microscopic behaviour modelling of a huge inverse problem non-trivial geometry
Numerical simulation of the biomechanical action of the diaphragm during respiration or ventilation is a challenging problem. The shape of the diaphragm is non-trivial and there are gradual transitions between muscle and tendon with very different material response. Imperfect data can be extracted from medical images, and can then be converted into a geometry representation~\cite{invive}. The specific challenges of constructing a smooth geometry representation are addressed in a 
forthcoming paper~\cite{Larsson20}. 

%The thickness of a human diaphragm is only around 5 mm, while the length along the surface is around 500 mm. That is, we have a large aspect ratio and with a uniform discretization it is expensive to resolve the thickness.

%The constitutive relations of muscle tissue are generally assumed to be non-linear and the displacements during respiration are large. Furthermore, there is uncertainty in what model and constitutive parameters best describes the diaphragm. The loss of muscle function during VIDD depends on miscroscopic properties. To understand this process a multiscale model, where macroscopic properties are computed from a microscopic simulation of a small tissue segment as in~\cite{Coelho18}, is needed.

In this paper, we model the diaphragm using a linear elastic PDE. This is a simplification and we plan to develop 
a more realistic tissue model as a part of our future work.

The boundary conditions for the elastic PDE system are given by a combination of traction boundary conditions, 
which contains first derivatives of the displacement, and (time-dependent) Dirichlet boundary conditions for the displacement, 
where the diaphragm is attached. These are mixed boundary conditions, in general not fully compatible, 
leading to reduced regularity of the solution even when we expect a smooth solution 
from a physiological perspecitve. 
Therefore, we smooth the boundary data as well as the transition between the traction boundary data and Dirichlet 
boundary data before using it in the PDE solver. 
%From a modelling perspective, it is hard to determine how large the attachment area is, 
%and exactly where the lungs exert pressure on the diaphragm. 
%The application of smoothed boundary conditions for linear elastic problems is studied in another forthcoming publication~\cite{smoothedbcs}.
% Non-trivial geometry.
% Anisotropy
% Non-linear equations
% Unknown modell
% VIDD microscopic properties
% Boundary conditions pressure relations
% We address some of these here

%--------------------------------------------------------------------------
% WHO have worked on this before and HOW
% Maybe the need for fast comes here.
% ends with our previous work. We are going to need to cite the smoothing paper. Will we cite/use the geometry paper? We should at least cite it. Then we describe what the aims are and that data is medical and all this.
% Cite the INVIVE project.

We use the unfitted radial basis function generated finite difference method in the least-squares setting 
(unfitted RBF-FD-LS)~\cite{tominec2020unfitted} to solve the diaphragm problem. A benefit of using the unfitted RBF-FD-LS method is that the PDE problem 
is solved on an extended domain (see Figure \ref{fig:method:diaphragm_interpNodes}). This simplifies node generation 
as the node placement is then independent of the geometry.
Another benefit of the unfitted setting is a smaller approximation error near the boundaries \cite{tominec2020unfitted}, where the stencils 
are typically highly skewed when using conventional RBF-FD methods such as the fitted RBF-FD-LS method \cite{ToLaHe20} 
and the collocation RBF-FD method \cite{FoFly15book}. 

As model geometry we use a two-dimensional cross section of the diaphragm.
To investigate the properties of the problem we use a combination of data from medical images and knowledge about the physiology of the diaphragm 
expressed in terms of boundary conditions. In particular, we construct two benchmark problems: (i) a pure Dirichlet case, (ii) 
a case with mixed boundary conditions (Dirichlet + traction), rephrased as a Robin condition with smooth coefficients.
With the experiments performed for these benchmarks, we aim to answer the following questions:
\begin{itemize}
\item Can we solve the benchmarks problems with unfitted RBF-FD-LS? Are there specific numerical challenges to be noted?
\item Can we achieve high-order convergence to the solution of the elastic PDE when the imposed boundary data and the geometry is smooth?
\item How is the performance and accuracy of the RBF-FD-LS solver affected by the type of boundary conditions that are imposed?
\item How does the RBF-FD-LS solver compare with a basic FEM solver? Do the solvers give similar solutions?
\end{itemize}

\new{Other authors have also modeled the diaphragm numerically.} The most advanced diaphragm simulations in the literature can be found in a series of publications by Ladjal et al.~\cite{Ladjal13,Ladjal15,Ladjal15b,Giroux17,Ladjal19}. The application focus is to track the motion of lung tumours during respiration for radiotherapy purposes. The finite element models that are employed are highly elaborate, taking into account features such as patient-specific lung compliance in order to define the constitutive law. 
The simulation times reported are far from real-time capability. In these studies, the diaphragm is not the main target and it  is not well-resolved in the thickness direction due to the high aspect ratio.
%
% Other simulations
Other relevant, but less detailed, diaphragm simulations can be found in~\cite{Pato11}, where the diaphragm is discretized using shell elements to compare healthy and pathological situations, and in~\cite{Fuerst14}, where the whole region under the lungs, including the diaphragm, forms one region in the simulation.

%Other diaphragm simulations can be found in the literature that are not focusing on the accuracy but on the computing time. In~\cite{villard09}, a tensegrity framework is developed. The organ is composed of mass-spring elements for the muscle part and a combination of rigid elements and mass-spring elements for the tendon part. It reproduced the global expected behavior but is not as accurate as a fully mechanical-based simulation. An even faster method is used in~\cite{bello09}: the chainmail method. It is a heuristic method where geometrical constraints simulate the mechanical action of compression, tension and shear. There is no PDE to solve so the computing time allows the 500Hz speed necessary to do haptic rendering.


%In both~\cite{Ladjal15b} and~\cite{Fuerst14}, image data is employed for tuning the muscle strength parameters for individual patients. The muscle parameters are given at the macro level.
%It would be difficult to calibrate a detailed model in the same way.
%In our project, apart from calibration to patient data, we are also interested in prediction of ventilator response based on physiological parameters such as, e.g., fat content and muscle fiber size~\cite{Cacciani14}, which affects the muscle tissue on a microscopic level. In this context, the thesis~\cite{Coelho18} is an interesting example of multiscale diaphragm modeling, where macroscopic properties are computed from a microscopic simulation of a small tissue segment.%, where the composition of the tissue can be varied.

% Interesting for patient-specific micro-properties.

%\begin{figure}[!htb]
%  \centering
%  \includegraphics[width=0.3\textwidth]{../Prof17/diacyl.jpg}
%  \includegraphics[width=0.3\textwidth]{/home/bette/Dropbox/Talks/Banff19/zintersect.png}
%  \includegraphics[width=0.3\textwidth]{/home/bette/Dropbox/Talks/Banff19/smoothedmesh.png}
%  \caption{\small\it The adaptive division of the diaphragm geometry (upside down) into overlapping cylinders, level set curves in an intersection of the domain, and a close up of the initial mesh (black) and the smoothed level set curves.}
%  \label{fig:1}
%\end{figure}

%During the INVIVE project, we have until now made two significant methodological contributions. The first is the least-squares RBF-PUM method~\cite{LaShchHer17}. It has practical advantages, such as using template node sets in the patches, which speeds up computation, and reduces node generation to the task of finding one good node set in a simple shape. The most important property, however, is that it is numerically stable under patch refinement, which is not true for collocation RBF-PUM. This makes it possible to solve large scale application problems.

%The second contribution is the least-squares RBF-FD method~\cite{ToLaHe20}, which similarly is stable under node refinement, and performs significantly better than collocation-based RBF-FD in the presence of Neumann boundary conditions. As far as we know, this is the first time that a complete proof of approximation stability has been constructed for the RBF-FD method in a general setting. A recent preprint~\cite{Davydov19} provides theoretical results for a different form of least-squares RBF-FD, restricted to a closed manifold.

%Both of these methods are well suited for the diaphragm problem and will be used as components in our virtual patient simulations.
%--------------------------------------------------------------------------

% WHAT are we going to do about it
% this includes simplifications that we make
% Proof of concept, what are we studying? How is the nuemrical method affected by different modelling aspects.

% OUR IDEA RBF-methods, and here LS-RBF-FD for smooth problems.
% Some preliminary results in invive.
% Some RBF-FD-LS with smoothed BCs in smoothedbcs for model problems. How to choose the parameters.
% What is different here?  We use the method and the bc technique to solve the diaphragm problem. Real data physiological behaviour.
% sensitivity to the implementation of boundary conditions. Anisotropy?
% This is one of the things we want to learn.
% How does the solution to the elastic problem behave?
% Our idea is to use localized radial basis function (RBF) methods, such as RBF-generated finite difference methods (RBF-FD)~\cite{FoFly15book} and RBF partition of unity methods (RBF-PUM)~\cite{LaShchHer17} to simulate the diaphragm. 
% These methods can easily be made high-order in general geometries, and are furthmore not bound to grid-based node layouts. 
% We expect the displacement of the real diaphragm to be smooth, and we use the smoothed boundary condition approach from~\cite{smoothedbcs} to ensure that also the numerical solution is smooth. 
% Some preliminary results for a linear elastic problem in the diaphragm geometry solved using RBF-FD are found in~\cite{invive}. 
% In these experiments, to have convergence, we needed to resolve the thickness direction of the diaphragm. 

% Collocation RBF-FD methods have been observed to have some robustness issues in the presence of Neumann boundary conditions~\cite{LiKeChu06,ToLaHe20}. 
% The least squares RBF-FD method (RBF-FD-LS) introduced in~\cite{ToLaHe20} is shown to have improved stability properties and is shown to perform well for Poisson problems with mixed boundary condition. 
  
The outline of the paper is as follows: Section~\ref{section:diabehavior}
describes the expected behavior of the diaphragm during respiration and the relation of the two-dimensional 
geometry to the real three-dimensional diaphragm geometry. 
Then the linear elasticity model problem is defined in Section~\ref{sec:linearelasticity}. 
An RBF-FD algorithm for computing differentiation and evaluation matrices is described in Section~\ref{sec:rbffd}. 
In Section~\ref{sec:unfitted_discretization} these matrices are then used in the least-squares unfitted RBF-FD setting 
to discretize the linear elasticity equations.
Section ~\ref{sec:smooth} discusses how the boundary of the two-dimensional diaphragm cross-section, and the boundary conditions, are smoothed. 
In Section ~\ref{sec:experiments:dirichlet} and Section~\ref{sec:experiments:Robin} we compute the solution to the linear elasticity equations 
for the two benchmark problems, and evaluate the convergence numerically. 
Finally, Section~\ref{sec:conclusions} contains the conclusions.


==> sections/2_diaphragm_respiratory.tex <==
\section{The expected behavior of the thoracic diaphragm}
\label{section:diabehavior}
The diaphragm is a musculotendinous structure, approximately double-dome shaped, separating the thoracic and abdominal cavities.  
It is the main muscle of the physiological respiration,  performing 70--80\% of the work of breathing, although it also has non-ventilatory functions, e.g., coughing, hiccups, sneezing, vomiting, and postural functions. It is composed  of three main parts, see Figure~\ref{fig:1a}. 
There are two muscular parts, one median and horizontal in upright position,  separating the thoracic and the abdominal organs, and another lateral muscle 
part, which ends with the costal insertions (attachment to the lower ribs), and there is one central tendon, where the extremities of all the muscle fibers converge. When the diaphragm contracts 
during inspiration (inhalation) with a piston-like motion, the muscle zone thickens (inspiratory thickening), and the domes move caudally (downward) expanding the thorax. Therefore, the air enters the lungs under a pressure gradient, see Figure~\ref{fig:1b}.
%
% It is acting like a pump to fill the lungs that are on its top with air. It is composed of a tendinous part on the top that is very stiff and a muscle par that is more elastic (see Figure \ref{fig:diaphAnatomy}.a). The diaphragm is also attached to the floating ribs in the appositional zone. The ribs are stretching the diaphragm when rotating through the action of the intercostal muscles \cite{Wilson}. When the diaphragm is contracting its muscle part, the tendinous part is almost performing a translation movement downward. It is an isotonic contraction:  the muscle decreases the length and consequently the thickness increases, because of the overlapping of the filaments in the sarcomeres \cite{}.
%
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[height=0.55\textwidth]{pics/intro/anatomyDiaph1.pdf}
    \caption{\textbf{Expiration state} with anatomical part}
    \label{fig:1a}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[height=0.55\textwidth]{pics/intro/anatomyDiaph2.png}
    \caption{\textbf{Inspiration state} with muscle actions}
    \label{fig:1b}
  \end{subfigure}
  \caption{Anatomy and physiology of the diaphragm (red and green parts) from expiration
to inspiration}
  \label{fig:diaphAnatomy}
\end{figure}

The two-dimensional geometry used for our simulations was extracted from a real patient medical image.
We used a 3D CT scan image (resolution: $0.927 \times 0.927 \times 0.3$ mm$^3$) that was acquired for medical reasons, see our previous work~\cite{invive}. The diaphragm was manually segmented in 3D following visual cues as explained in \cite{villard11}. The labeled voxels were exported to a triangle mesh with the Marching Cube algorithm and the mesh was simplified with a decimation algorithm \cite{levy2010}.

The frontal plane slice we selected is in the middle of the body, corresponding roughly to the anatomic illustration of Figure~\ref{fig:diaphAnatomy}. The raw data consists of a list of 2D vertices where a topology can easily be extracted.
%and the information of which points belong to the thorax or to the abdomen could be found as well.
The raw geometry data contains noise from several sources.
There is some CT scan device incertitude (noise, calibration etc) \cite{Zatz77}, the data is the result from a discretized process,  and the labeling data comes from a manual segmentation that is prone to human error. Concerning this last point, the diaphragm is not entirely visible, sometimes part of its voxels also include other organs. The accuracy is linked to the imagination and the anatomical knowledge of the medical expert that performed the segmentation.

%
% The expected displacement between relaxed and contracted state
% In the slice
The expected displacement of the diaphragm between the relaxed and contracted states in the two-dimensional slice is is roughly illustrated in Figure~\ref{fig:smoothing:bcPosition}. For the numerical simulations in Sections~\ref{sec:experiments:dirichlet} and~\ref{sec:experiments:Robin}, we construct boundary conditions to replicate this motion qualitatively.
\begin{figure}[h!]
\centering
\includegraphics[width=0.85\linewidth]{pics/smoothing/BCs.png}
\caption{The expected displacement in different parts of the slice of the diaphragm. The red areas correspond to the real physiological behavior and the green areas are transition zones. In regions 3 and 7, there is both a thickening of the muscle and a downward motion, while in region 5, the downward motion dominates.}
\label{fig:smoothing:bcPosition}
\end{figure}


%The displacements have been synthesized to reproduce the physiological behavior described in Section 
%\ref{section:diabehavior}. Particularly, the translation motion of the tendon has been defined by a constant displacement 
%in the superior to inferior direction ($x$ direction) and the thickening of the appositional zone is also done in the lateral direction ($y$ direction)
%in the same way. 


==> sections/2_medicalContextAndImageProcessing.tex <==
\section{The diaphragm as a part of the respiratory cycle}
\label{section:diabehavior}
The diaphragm is a musculotendinous structure, approximately double-dome shaped, separating the thoracic and abdominal cavities.  
It is the main muscle of the physiological respiration  performing the 70-80\% of the Walk of Breathing, although it also has non ventilatory functions 
(e.g. cough, hiccup, sneeze, vomiting, postural functions). It is composed  of 3 main parts  (see Figure \ref{fig:diaphAnatomy}.a). 
Two muscular parts, one median and horizontal in upright position,  separating the thoracic to the abdominal organs and another lateral muscle 
part which ends with the costal insertions; one central tendon, where the extremities of all the muscle fibers converge. When the diaphragm contracts 
during the inspiration with a piston-like motion, the muscle zone thickens (inspiratory thickening), so the domes move caudally expanding the thorax, 
therefore the air enters the lungs under a pressure gradient (see Figure \ref{fig:diaphAnatomy}.b).

% It is acting like a pump to fill the lungs that are on its top with air. It is composed of a tendinous part on the top that is very stiff and a muscle par that is more elastic (see Figure \ref{fig:diaphAnatomy}.a). The diaphragm is also attached to the floating ribs in the appositional zone. The ribs are stretching the diaphragm when rotating through the action of the intercostal muscles \cite{Wilson}. When the diaphragm is contracting its muscle part, the tendinous part is almost performing a translation movement downward. It is an isotonic contraction:  the muscle decreases the length and consequently the thickness increases, because of the overlapping of the filaments in the sarcomeres \cite{}.


\begin{figure}
    \centering
    \begin{tabular}{cc}
        \includegraphics[height=5cm]{pics/intro/anatomyDiaph1.pdf} & \includegraphics[height=5cm]{pics/intro/anatomyDiaph2.png} \\
        \textit{a) \textbf{Expiration state} with anatomical part}s & \textit{b) \textbf{Inspiration state} with muscle actions}
    \end{tabular}
    \caption{Anatomy and physiology of the diaphragm (red and green parts) from expiration to inspiration}
    \label{fig:diaphAnatomy}
\end{figure}


The geometry used for our simulation was extracted from a real patient medical image.
We obtained a 3D CT scan image (resolution: $0.927 \times 0.927 \times 0.3 mm^3$) that was acquired for medical reasons as explained in our previous work (see \cite{invive}). The diaphragm was manually segmented in 3D following visual cues as explained in \cite{villard11}. The labeled voxels were exported into a triangle mesh with the Marching Cube algorithm and the mesh was simplified with a decimation algorithm \cite{levy2010}.

The slice in the frontal plane was selected in the middle corresponding roughly to the anatomic illustration of Figure~\ref{fig:diaphAnatomy}. These raw data consist of a list of 2D vertices where a topology could easily be extracted and the information of which points belong to the thorax or to the abdomen could be found as well. However, the data are not smooth for various reasons:
i) there is some CT scan device incertitude (noise, calibration etc) see \cite{Zatz77}, ii) they result from a discretized process  and iii) the labeling data results from manual segmentation that are prone to human error. Concerning this last point, the diaphragm is not entirely visible, sometime part of its voxels also include other organs. 
It is linked to the  imagination and the anatomical knowledge from the medical expert that did the segmentation.

==> sections/3_elasticity.tex <==
\section{Equations of linear elasticity}
\label{sec:linearelasticity}
The simplified model that we use is valid for studying 
small deformations of an isotropic and homogenuous diaphragm with a linear elasticity constitutive law. 
The deformation of a diaphragm $\Omega$ is described by applying a displacement field $ u = (u_1, u_2)^T,$ to an object 
location $ y = (y_1, y_2)^T \in \Omega$ such that:
$$ y^* =  y +  u,$$
where $ y^* = (y_1^*, y_2^*)^T \in \Omega^*$ is then a deformed object.
A field derived from the displacements is the stress tensor: 
$$\usigma = \begin{pmatrix}\sigma_{11}& \sigma_{12} \\ \sigma_{21}& \sigma_{22} \end{pmatrix},$$
which measures the internal forces in $\Omega$ as a consequence of deformation. It is related to the displacement field by: 
\begin{equation}
    \label{eq:model:stressAndStrain}
\usigma = \lambda \Tr(\uvarepsilon) + 2\mu\uvarepsilon,\qquad    
    \uvarepsilon = \frac{1}{2}\left( \left(\nabla u\right)^T + \nabla  u \right),
\end{equation}
where $\uvarepsilon\in\mathbb{R}^{2\times 2}$ is the strain tensor and $\Tr(\uvarepsilon) = \left(\varepsilon_{11} + \varepsilon_{22}\right)I$ is its trace. 
The scalars $\lambda$ and $\mu$ are the Lam\'e parameters, which are related to the Young modulus $E$ and the Poisson ratio $\nu$ of the material through:
\begin{equation}
    \label{eq:model:lame}
    \lambda = \frac{E\nu}{\left(1+\nu\right)\left(1-2\nu\right)},\qquad 
    \mu = \frac{E}{2\left(1+\nu\right)}.
\end{equation}
For our computations 
we use $E=10^5\, \text{Pa}$ and $\nu = 0.3$.
A special stress measure that is also of interest to us is the Von Mises stress:
\begin{equation}
    \label{eq:model:vonMises}
\sqrt{\sigma_{11}^2 - \sigma_{11}\sigma_{22} + \sigma_{22}^2 +  3\sigma_{12}^2},
\end{equation}
which provides a scalar measure of the total stress.

The equations of linear elasticity are derived from the force equilibrium (Newton's second law) imposed on $\Omega$. 
We have:
\begin{equation}
\begin{aligned}
\label{eq:model:secondNewton}
- \nabla \cdot \usigma =  f \text{ on } \Omega,
\end{aligned}
\end{equation}
where $ f = \left(f_1( y), f_2( y)\right)^T$ is a field of 
internal forces in the horizontal and the vertical direction.
The Dirichlet and traction boundary conditions are prescribed on two disjoint parts of the 
boundary, which together form the whole boundary $\partial\Omega = \partial\Omega_0 \cup \partial\Omega_1$:
\begin{equation}
    \begin{aligned}
\label{eq:model:secondNewton_bcs}
 u &=  g \text{ on } \partial\Omega_0, \\
\usigma \cdot  n &=  h \text{ on } \partial\Omega_1.
    \end{aligned}
\end{equation}
The first boundary condition with the right hand side $ g = \left(g_1( y), g_2( y)\right)^T$ is the displacement 
condition. 
The second boundary condition with the right hand side $ h = \left(h_1( y), h_2( y)\right)^T$ is the traction condition. 
An equivalent form of \victor{\eqref{eq:model:secondNewton_bcs}} is the Robin boundary condition:
\begin{equation}
\begin{aligned}
    \label{eq:model:secondNewton_bcs_Robin}
     u\, \kappa_0(y)  +  \left(\usigma \cdot  n\right)\, \kappa_1(y) =   g\, \kappa_0(y) +   h\, \kappa_1(y)  \text{ on } \partial\Omega = \partial\Omega_0 \cup \partial\Omega_1,
\end{aligned}
\end{equation}
where $\kappa_0$ and $\kappa_1$ correspond to two spatially dependent coefficients, in this case discontinuous: 
$\kappa_0(y) = 1$ when $y\in \victor{\partial} \Omega_0$ and zero otherwise, and $\kappa_1(y) = 1$ when $y\in \victor{\partial}\Omega_1$ and zero otherwise.

\victor{In Section \ref{sec:experiments:dirichlet}} we first compute solutions using a Dirichlet condition for the whole boundary. 
($\kappa_0(y) = 1$, $\kappa_1(y)=0$, $y \in \partial \Omega$). 
Then, \victor{in Section \ref{sec:experiments:Robin}}, we compute 
solutions using smoothed Dirichlet and traction conditions (smooth Robin coefficients), which approximates the 
imposition of these two conditions on two disjoint parts of the diaphragm. However, since physiology suggests a smooth solution, 
we see this as modeling rather than as an error.


%\subsection{The Navier-Cauchy system of equations}
%\label{sec:model:naviercauchy}
For all of the computations in this paper we use the displacement formulation of \eqref{eq:model:secondNewton}, obtained by 
using the relation between stress and displacement  given in \eqref{eq:model:stressAndStrain}. The force equilibrium 
\eqref{eq:model:secondNewton} then expands to:
$$- \nabla \cdot \usigma = - \mu \nabla^2 {u} - (\lambda + \mu)\nabla (\nabla \cdot {u}) =  f,$$
and the traction boundary condition from \eqref{eq:model:secondNewton_bcs} to:
$$\usigma \cdot  n = \left[\lambda \left(\nabla \cdot  u \right)I + \mu \left(\left(\nabla  u\right)^T + \nabla  u\right)\right] \cdot  n =  h.$$
The displacement formulation of the linear elasticity equations with the boundary condition from \eqref{eq:model:secondNewton_bcs_Robin} 
is then written as:
\begin{equation}
\begin{aligned}
    \label{eq:model:naviercauchy}
- \mu \nabla^2 u - (\lambda + \mu)\nabla (\nabla \cdot u) = &\, f  &\text{ on } \Omega,& \\
u\, \kappa_0 + \left(\left[\lambda \left(\nabla \cdot  u \right)I + \mu \left(\left(\nabla  u\right)^T + \nabla  u\right)\right] \cdot  n \right)\kappa_1 = &\, g\, \kappa_0 + h\, \kappa_1 & \text{ on } \partial\Omega&.
\end{aligned}
\end{equation}
For simplicity we rewrite the system above as:
$$Du(y) = F(y),$$ 
where:
\begin{equation}
\begin{aligned}
    \label{eq:model:PDE}
    D u( y) &=
    \left\{
    \begin{array}{ll}
        D_2  u( y), &  y \in \Omega \\
        \kappa_0( y) D_0  u( y) + \kappa_1( y) D_1  u( y) \cdot  n( y), &  y \in \partial\Omega
    \end{array}
    \right. & %\,
    \\
    F(y) &=
    \left\{
    \begin{array}{ll}
         f( y), &  y \in \Omega  \\
         \kappa_0( y) g( y) + \kappa_1( y) h( y), &  y \in \partial\Omega
    \end{array}
    \right. &
\end{aligned}
\end{equation}
Here $D_2$, $D_1$, $D_0$ are the expanded operators that in \eqref{eq:model:PDE} correspond to 
$\Omega$, $\partial\Omega_1$ and $\partial\Omega_0$ respectively. If we let $\nabla_{ij}=\frac{\partial^2}{\partial y_i\partial y_j}$ and  $\nabla_i=\frac{\partial}{\partial y_i}$, then the operator $D_2$ is:
\begin{equation}
\label{eq:model:PDE_D_2}
D_2 
= 
-
\begin{pmatrix}
(\lambda+2\mu)\nabla_{11} + \mu \nabla_{22} & (\lambda + \mu) \nabla_{12} \\
(\lambda + \mu) \nabla_{12} & \mu \nabla_{11} + (\lambda+2\mu) \nabla_{22}
\end{pmatrix},
\end{equation}
and the boundary operators $D_1$ and $D_0$ are:
\begin{equation}
\label{eq:model:PDE_D_1_0}
D_1 
= 
\begin{pmatrix}
\mu n_2 \nabla_2 + \left(\lambda + 2\mu\right) n_1 \nabla_1 & \lambda n_1 \nabla_2 + \mu n_2 \nabla_1 \\
\mu n_1 \nabla_2 + \lambda n_2 \nabla_1 & (\lambda+2\mu)n_2\nabla_2 + \mu n_1 \nabla_1
\end{pmatrix}, \quad 
D_0 
=
\begin{pmatrix}
I & 0 \\ 0 & I
\end{pmatrix}.
\end{equation}



==> sections/4_functionSpace.tex <==
\section{Approximation of functions using the RBF-FD method}
\label{sec:rbffd}
Here we describe the approximation framework which is used when representing the unknown displacement and the 
stress (which are the outputs of the simulation), and the known data vectors (the input data to the simulation) as continuous functions. 
The following discussion is general in the sense that 
the data vector can be known or unknown. Concrete examples of using the framework developed in this section are given 
in later sections.

Given a data vector $\tilde u(X) = [\tilde u(x_1), \tilde u(x_2), ..., \tilde u(x_N)]^T$ where $x_i \in \mathbb{R}^d$ 
we construct a semi-discrete evaluation operator $E=E(y,X)$, which, for 
any point $y \in \Omega \subset \mathbb{R}^d$, returns the value of the interpolant of the data $\tilde u(X)$ at that point, 
such that:
\begin{equation}
    \label{eq:rbffd:evaluation}
\tilde u(Y) = E(y,X) \tilde u(X).
\end{equation}
Now we use \eqref{eq:rbffd:evaluation} for each $y \in Y$ to obtain a system of equations and form the matrix 
$E(Y,X)$ of size $M \times N$, $M \geq N$. Note that in our notation this is equivalent to setting $y=Y$.
The RBF-FD procedure constructs the matrix $E(Y,X)$ using a sequence of local, stencil-based interpolation problems 
which are exact for a cubic or quintic polyharmonic spline basis (PHS) and a (multivariate) monomial basis of degree $p$.
The matrix $E(Y,X)$ is sparse, that is, 
it contains $n \ll N$ non-zero elements per row, where $n$ is the stencil size defined by:
\begin{equation}
\label{eq:rbffd:stencilsize}
n = 2\,\binom{p+d}{d}.
\end{equation}
Details about using PHS plus the monomial basis in RBF-FD approximations can be found in \cite{BFFB17, BFF19, Bayona19, Barnett15}.
\victor{In the same way,} we construct a semi-discrete oprator for differentiation $D^{\mathcal{L}} = D^{\mathcal{L}}(y,X)$ which locally evaluates any 
derivative $\mathcal{L}$ of $\tilde u(Y)$:
\begin{equation}
    \label{eq:rbffd:differentiation}
    \mathcal{L} \tilde u(Y) = D^{\mathcal{L}}(y,X) \tilde u(X).
\end{equation}

\victor{Both matrices, $E(Y,X)$ and $D^{\mathcal{L}}(Y,X)$, can be formed using the MATLAB code available in \cite{tominec_rbffdcode}.} 
\victor{For completeness, we below provide the steps to compute the matrix elements (weights) and to assemble 
$D^{\mathcal{L}}(Y,X)$ and $E(Y,X)$ 
for the point sets $Y$ and $X$ in any dimension $d$.}
\begin{enumerate}
    \item Let $x_1^{(k)} = x_i \in X$ (one stencil center) and find 
    $n$ closest neighbors $\left\{x^{(k)}_j\right\}_{j=1}^n$ (stencil points) around it using the Euclidean distance.
    \item Scale and shift the stencil points to a unit domain $[-1,1]^d$. \victor{Save the scaling as $s^{(k)}$.}
    \item Form a square interpolation matrix $A^{(k)}$, where $A^{(k)}_{ij}=r^3=||x_i^{(k)}-x_j^{(k)}||_2^3$ 
    \victor{and $x_i^{(k)},x_j^{(k)},\, i,j = 1,..,n$ belong to the stencil}.
    \item Form a rectangular polynomial matrix $P^{(k)}$, where $P^{(k)}_{il} = p_l(x_i^{(k)})$, $i=1,..,n$, $l=1,..,m$ is a sampled $d$-dimensional monomial basis 
    with $m$ basis functions.
    \victor{When $n$ is chosen as in \eqref{eq:rbffd:stencilsize} 
    then $m = \frac{n}{2}$ and the size of the matrix $P^{(k)}$ is $n \times \frac{n}{2}$.}
    \item Using $A^{(k)}$ and $P^{(k)}$, form the augmented local interpolation matrix:
    \begin{equation}
	    \label{eq:M}
	    \tilde{A}^{(k)} = \begin{pmatrix}
		    A^{(k)} & P^{(k)} \\
	    	(P^{(k)})^{T} & 0
	    \end{pmatrix}
    \end{equation}
    
    \item Repeat steps 1--5 for every $x \in X$ in order to form all $\tilde{A}^{(k)}$.
\end{enumerate}
The local evaluation and differentiation weights can then be computed in the following way:
\begin{enumerate}    
    \item Take one evaluation point $y_l \in Y$ and find the first closest point from the $X$ point set. We denote it by $x_1^{(k)}$.
    \item Scale $y_l$ to a unit domain $[-1,1]^d$ \victor{using the previously computed scaling $s^{(k)}$}.
    \item Form a vector $b_1 = \mathcal{L}||y_l-x^{(k)}_j||_2^3$, where $\{x^{(k)}_j\}_{j=1}^{n}$ is the local neighborhood of the 
    center point $x_1^{(k)}$, \victor{where $\mathcal{L} = 1$ for constructing evaluation weights, or a derivative operator for constructing differentiation weights.}
    \item Form a vector $b_2 = \mathcal{L} p_j(y_l),\, j=1,..,\frac{n}{2}$.
    \item Concatenate the two vectors into $b(y_l) = [b_1,\, b_2]$.
    \item Use the augmented interpolation matrix that belongs to $x_1^{(k)}$ and compute the local weights by using the relation 
    $w_{\mathcal{L}}(y_l) = (\tilde{A}^{(k)})^{-1} b_{\mathcal{L}}(y_l)$.
    \item Store $w_{\mathcal{L}}(y_l)$ in the $l$-th row of the matrix $W_{\mathcal{L}}(Y)$.
    \item Repeat steps 1--6 for every $y_l \in Y$ in order to form all local weights.
\end{enumerate}
\victor{When using these steps to compute the weights, it is possible to avoid storing the matrix 
$\tilde{A}^{(k)}$ by combining the two parts such that the evaluation/differentiation weights are computed for all $y_l$ 
which select $x_1^{(k)}$ as its closest stencil center, immediately after step 5 of the first list.}
Once the matrix of local weights $W_{\mathcal{L}}(Y)$ of size $M \times n$ is computed, 
these weights are assembled into a global rectangular matrix, $E(Y,X)$ for evaluation and 
$D_{\mathcal{L}}(Y,X)$ for differentiation, both of size $M \times N$. This can be done by using a matrix $\Gamma \in \mathbb{Z}^{N\times n}$, 
which is a list of indices of the local neighborhoods of points around every stencil point $x_1^{(k)} \in X$. 
Additionally, a matrix $\kappa \in \mathbb{Z}^{M\times 1}$ is needed, which is a list of indices of the 
stencil centers that are closest to each evaluation point $y_l$. $\Gamma$ and 
$\kappa$ are found using the k-nearest neighbor method with $k$ equal to $n$ and $1$, respectively.
Using the MATLAB programming language, the two lists and the sparse matrix can be efficiently computed by 
invoking the following three commands:
\begin{verbatim}
    Gamma = knnsearch(X,X,'k',n)
    kappa = knnsearch(X,Y,'k',1)
    D_L = sparse(repmat(1:M, 1, n), Gamma(kappa,:), W_L, M, N, N*n)
\end{verbatim}
where the first two arguments to the function \texttt{sparse()} have the same shape as $W_{\mathcal{L}}(Y)$ 
and contain the row and column indices for inserting the locally computed weights into the global matrix.
%A complete MATLAB code for computing differentiation matrices as described above is provided in \cite{tominec_rbffdcode}.


==> sections/5_pdemethod.tex <==
\section{Discretization of the linear elastic model using the uniftted RBF-FD method}
\label{sec:unfitted_discretization}
In this section we employ the unfitted RBF-FD method \cite{tominec2020unfitted} to discretize the linear elasticity equations 
\eqref{eq:model:PDE}, \eqref{eq:model:PDE_D_2} and \eqref{eq:model:PDE_D_1_0} over the diaphragm. 
The method relies on constructing rectangular 
differentiation matrices $D^\mathcal{L}(Y,X)$ as described in 
Section \ref{sec:rbffd}. The matrices then replace the differential operators in the PDE, together with the corresponding 
discrete right hand sides $F(Y)$.

To form the differentiation matrices, we first decide the degree $p$ of the monomial basis that we are appending to the 
PHS approximation, and compute the stencil size $n$ using \eqref{eq:rbffd:stencilsize}.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{pics/Domain/diaphragma_noVoronoi.pdf} 
    \caption{The initial point set $X_1$ (tilted Cartesian points) is distributed over a box that encloses the boundary 
    of the diaphragm (black curve). Points that are more than half a stencil size away from the geometry (grey) are removed. 
    The remaining points (blue) form the point set $X$.}
    \label{fig:method:diaphragm_interpNodes}
\end{figure}
Then we construct an interpolation point set $X$ 
that extends over the diaphragm (see Figure \ref{fig:method:diaphragm_interpNodes}), and an 
evaluation point set $Y$ (see Figure \ref{fig:method:diaphragm_evalNodes}) that conforms to the geometry of the diaphragm. 
Those two point sets are obtained in four simple steps:
\begin{itemize}
\item The initial point set $X_1$ is a tilted Cartesian node layout with spacing $h$ in a box that 
encloses the diaphragm. \victor{(the grey and blue points in Figure \ref{fig:method:diaphragm_interpNodes})}.
\item Then the point set $Y_1$ is generated by placing $q$ points with average spacing $h_y$ in each Voronoi region inside the diaphragm, 
defined by the points in $X_1$. \victor{(the red points in Figure \ref{fig:method:diaphragm_evalNodes})}.
\item In addition, the point set $Y_b$ with the same average spacing $h_y$ is generated by placing points 
along the boundary of the diaphragm, see Figure \ref{fig:method:diaphragm_evalNodes}.
\item The final evaluation point set is given by $Y = Y_1 \cup Y_b$, see Figure \ref{fig:method:diaphragm_evalNodes}.
\item The final node set $X$ (the blue points in Figure \ref{fig:method:diaphragm_interpNodes} and Figure \ref{fig:method:diaphragm_evalNodes}) 
is formed by reducing $X_1$ by removing points that fall more than half stencil size outside the diaphragm. In Matlab this can be done by:
\begin{verbatim}
    X = X_1(unique(knnsearch(X_1,Y,’k’,ceil(0.5*n)), :);
\end{verbatim}
\end{itemize} 
The last step ensures that the columns of $E(Y,X)$ and $D^{\mathcal{L}(Y,X)}$ are non-zero \cite{tominec2020unfitted}. 
Note that the evaluation point set does not need to be constructed by placing precisely $q$ points in every Voronoi region. 
It is possible to use any 
global point set, which is quasi-uniform by nature (e.g. Halton points), 
and as such on average samples every Voronoi region with approximately $q$ points.
\begin{figure}[h!]
    \centering
\includegraphics[width=0.4\linewidth]{pics/Domain/diaphragma_Voronoi_unfitted_closeup.pdf}
    \caption{The black curve represents a part of the boundary of the diaphragm. 
    Node points in $X$ (blue markers) and the corresponding Voronoi regions (grey lines) are shown 
    together with interior evaluation points, $Y_1$, and boundary evaluation points, $Y_b$, (red markers). 
    The same template of interior evaluation points is used in each Voronoi region inside the diaphragm geometry.}
    \label{fig:method:diaphragm_evalNodes}
\end{figure}

%Now we subdivide the evaluation point set according to locations where the 
%interior and the boundary equations are imposed. In particular, 
%we can write that $Y_2 \subset Y$ is a set containing all points in the interior of the diaphragm, 
%and $Y_b \subset Y$ a set corresponding to the locations of the boundary of the diaphragm.
%We discretize the continuous operators $D_2$, $D_1$ and $D_0$ 
%given in \eqref{eq:model:PDE_D_2} and \eqref{eq:model:PDE_D_1_0} respectively. Then we replace the 
%continuous differential operators by the differentiation matrices introduced in Section \ref{sec:rbffd}

\elisabeth{%
Next, we use the method described in Section~\ref{sec:rbffd} to discretize the continuous operator $D_2$ in~\eqref{eq:model:PDE_D_2} using the interior evaluation points $Y_1$, and to discretize the continuous operators $D_1$ and $D_0$ in~\eqref{eq:model:PDE_D_1_0} using the boundary evaluation points $Y_b$. We let $D_k^{ij}(\,\cdot\,,X)$ denote the differentiation matrix that approximates element $i,j$, of the operator $D_k$, $k=0,\,1,\,2$. If we let $i,j=1,2$, while $i\neq j$, then we can express the differentiation matrices as:
  \begin{eqnarray*}
    D_2^{ii}(Y_1,X) &=& (\lambda+2\mu)D^{\nabla_{ii}}(Y_1,X) + \mu D^{\nabla_{jj}}(Y_1,X), \\
    D_2^{ij}(Y_1,X) &=& (\lambda + \mu) D^{\nabla_{ij}}(Y_1,X), \\
    D_0^{ii}(Y_b,X) &=& E(Y_b,X), \\
    D_0^{ij}(Y_b,X) &=& 0, \\
    %
    D_1^{ii}(Y_b,X) &=& (\lambda+2\mu)n_i D^{\nabla_i}(Y_b,X) + \mu n_j D^{\nabla_j}(Y_b,X),\\
    D_1^{ij}(Y_b,X) &=& \lambda n_i D^{\nabla_j}(Y_b,X) + \mu n_j D^{\nabla_i}(Y_b,X). \\
\end{eqnarray*}
}%
%\begin{eqnarray*}
%    D_2^{11} &=& D_2^{11}(Y_2,X) = (\lambda+2\mu)D^{\nabla_{xx}}(Y_2,X) + \mu D^{\nabla_{yy}}(Y_2,X) \\
%    D_2^{12} &=& D_2^{12}(Y_2,X) = (\lambda + \mu) D^{\nabla_{xy}}(Y_2,X) \\
%    D_2^{21} &=& D_2^{21}(Y_2,X) = D_2^{12} \\
%    D_2^{22} &=& D_2^{22}(Y_2,X) = \mu D^{\nabla_{xx}}(Y_2,X) + (\lambda+2\mu)D^{\nabla_{yy}}(Y_2,X)\\
%    D_0^{11} &=& D_0^{11}(Y_b,X) = E(Y_b,X) \\
%    D_0^{12} &=& D_0^{12}(Y_b,X) = 0 \\
%    D_0^{21} &=& D_0^{21}(Y_b,X) = D_0^{12} \\
%    D_0^{22} &=& D_0^{22}(Y_b,X) = E(Y_b,X) \\
%    D_1^{11} &=& D_1^{11}(Y_b,X) = \mu n_2 D^{\nabla_y}(Y_b,X) + \left(\lambda + 2\mu\right) n_1 D^{\nabla_x}(Y_b,X) \\
%    D_1^{12} &=& D_1^{12}(Y_b,X) = \lambda n_1 D^{\nabla_y}(Y_b,X) + \mu n_2 D^{\nabla_x}(Y_b,X) \\
%    D_1^{21} &=& D_1^{21}(Y_b,X) = \mu n_1 D^{\nabla_y}(Y_b,X) + \lambda n_2 D^{\nabla_x}(Y_b,X) \\
%    D_1^{22} &=& D_1^{22}(Y_b,X) = (\lambda+2\mu)n_2 D^{\nabla_y}(Y_b,X) + \mu n_1 D^{\nabla_x}(Y_b,X)
%\end{eqnarray*}
% Write the Robin conditions inline
% Du=F is same notation as continuous form. Never used later, therefore remove.
% Mention scaling before writing the system and then explain our choice after.
% hs should not be double sums.
\elisabeth{We express the discrete Robin coefficients as $K_i(Y_b) = \diag(\kappa_i(Y_b))$, $i=0,\,1$, and introduce a scaling $\beta_i$ for equations connected with the operator $D_i$.}
%\begin{equation}
%    \label{eq:method:Robincoeff}
%    K_0 = K_0(Y_b) = \diag(\kappa_0(Y_b)),\qquad\quad K_1 = K_1(Y_b) = \diag(\kappa_1(Y_b)).
%\end{equation}
%A rectangular system $D u = F$ of size $2M \times 2N$ is then a discretization of the Navier-Cauchy system~\eqref{} with 
% Robin boundary conditions~\eqref{}:
\elisabeth{Finally, we form the rectangular system of size $2M \times 2N$ that discretizes  the Navier-Cauchy system with 
 Robin boundary conditions~\eqref{eq:model:PDE}:}
 \begin{flalign}
   \small
   \label{eq:method:DandF}
    \begin{pmatrix}
        \beta_2\,D_2^{11} & \beta_2\, D_2^{12} \\
        \beta_2\, D_2^{21} & \beta_2\, D_2^{22} \\
        \beta_0\,K_0\, D_0^{11}+  \beta_1\,K_1\, D_1^{11}\hspace*{-2mm}& \beta_1\,K_1\, D_1^{12}\\    
        \beta_1\,K_1\, D_1^{21} & \hspace*{-2mm}\beta_0\,K_0\, D_0^{22} + \beta_1\,K_1\, D_1^{12} 
    \end{pmatrix}
%    u &= 
    \begin{pmatrix}
    \tilde u_1(X)\\
    \tilde u_2(X)
    \end{pmatrix}
    =
    %   ,\quad
    % F = 
    \begin{pmatrix}
        \beta_2\, f_1(Y_1)\\
        \beta_2\, f_2(Y_1)\\
        \beta_0\, K_0\, g_1(Y_b) + \beta_1\, K_1\, h_1(Y_b)\\
        \beta_0\, K_0\, g_2(Y_b) + \beta_1\, K_1\, h_2(Y_b)\\
    \end{pmatrix}.
\end{flalign}
 In the numerical experiments, we use the following scale factors:
% This is just scaling, not artificial scaling 
% where we additionally applied artificial scalings $\beta_2$, $\beta_1$, $\beta_0$ defined as:
\begin{equation}
    \beta_2 = \frac{1}{\mu}\, h_y,\quad \beta_1 = \frac{10}{\mu}\,\frac{1}{h}\, h_y^{\frac{1}{2}}, \quad \beta_0 = \frac{1}{h}\, h_y^{\frac{1}{2}},
\end{equation}
\victor{where $h$ and $h_y$ are the average internodal distances in the $X$ and $Y$ point sets, respectively. These are computed as:
%\begin{equation}
%    \label{eq:method:h_and_hy}
%h = \frac{1}{N} \sum_{i,j=1}^N \min_{x_i \neq x_j} \|x_i - x_j\|_2,\quad h_y = \frac{1}{M} \sum_{i,j=1}^M \min_{y_i \neq y_j} \|y_i - y_j\|_2.
  %\end{equation}
\begin{equation}
    \label{eq:method:h_and_hy}
h = \frac{1}{N} \sum_{j=1}^N \min_{i \neq j} \|x_i - x_j\|_2,\quad h_y = \frac{1}{M} \sum_{j=1}^M \min_{i \neq j} \|y_i - y_j\|_2.
\end{equation}
}%
%The scalings are based on papers \cite{tominec2020unfitted, ToLaHe20}, where $h_y$ and $h_y^\frac{1}{2}$ are applied 
%to the interior and the boundary equations separately, so that the discrete inner products correspond to 
%the continuous inner products plus a first order error term. The $1/h$ scaling is applied only to the boundary conditions. 
%An inverse of the large parameter $\mu$ is scaling the interior and the traction condition 
%to prevent large variations in the magnitude of different rows.
\new{The choice of scale factors is based on the papers \cite{tominec2020unfitted, ToLaHe20}, where the scale factors $h_y$ for the interior and $h_y^{1/2}$ for the boundary are used, such that the norms of the discrete least squares problem approximate the continuous $L_2$-norm. The additional $1/h$ scaling increases the weight of the boundary conditions and improves convergence. The Lam\'e parameter $\mu$ is large and affects the scaling between different equations. Therefore, we also include the factor $10/\mu$ in $\beta_1$.
}

We solve the least-squares problem \eqref{eq:method:DandF}, for the nodal values 
$\tilde u_1(X)$ and $\tilde u_2(X)$, using backslash in MATLAB. 
After that the solution is evaluated at the $Y$ point set, using the evaluation matrix $E$:
\begin{equation}
    \tilde u_1(Y) = E(Y,X)\, \tilde u_1(X),\, \qquad \tilde u_2(Y) = E(Y,X)\, \tilde u_2(X).
\end{equation}
The strains and the stresses \eqref{eq:model:stressAndStrain}, \eqref{eq:model:vonMises} are computed by applying appropriate 
differentiation matrices to the solution coefficients $\tilde u_1(X)$ and $\tilde u_2(X)$.



==> sections/6_boundaryCurve.tex <==
\section{A smooth representation of the diaphragm}
\label{sec:smoothDiaphragmBoundaryCurve}
In Section \ref{section:diabehavior} we explained how the initial point cloud of the boundary of the diaphragm was obtained from a 
CT scan. 
Here we transform this noisy boundary point cloud into a boundary curve.
At the end we obtain a parameterized reference boundary curve which is smooth and 
over which we can place points with an arbitrarily small internodal distance. All of these properties are important 
in order to make the simulation efficient. In particular, 
a larger degree of smoothness enables the error between the numerical solution and the exact solution of the model problem, 
to decay with a faster rate (high-order convergence). At the same time 
a smooth boundary curve makes the simulation physically more relevant.

The input data is a set of ordered data points in 2D which are first downsampled in size 
to make the final smooth curve less noisy. Throughout the paper we work with the boundary data that is from original locations 
scaled to a unit domain $[-1, 1]\times[-1,1]$.
The result is a set of coordinate pairs $\{(\tilde p_j, \tilde q_j)\}_{i=1}^M$.

\begin{figure}
    \label{fig:boundaryCurve:p_and_q_data_smooth}
    \centering
    \includegraphics[width=0.49\linewidth]{pics/smoothing/diaphragm_fit.pdf}
    \includegraphics[width=0.49\linewidth]{pics/smoothing/diaphragm_points.pdf}
\caption{Left: markers correspond to the input data points, the displayed red curve is the final smooth and periodic boundary of the diaphragm. Right: The displayed red curve 
is the final smooth and periodic boundary of the diaphragm and the markers placed on top represent a nearly equispaced point set over the boundary of the diaphragm. The arrows 
display a smooth distribution of the outward normals.}
\end{figure}

Then we compute parameter data $\tilde t_j$, which is the approximate arclength computed between the data points:
\begin{equation}
\begin{aligned}
    \label{eq:boundaryCurve:parameter}
    \tilde t_1(\tilde p_1, \tilde q_1) &=& 0 \\
    \tilde t_j(\tilde p_j,\tilde q_j) &=& \tilde t_{i-1} +  \sqrt{(\tilde p_j - \tilde p_{i-1})^2 + (\tilde q_j - \tilde q_{i-1})^2},\quad i=2,..,M
\end{aligned}
\end{equation}
The motivation to use the arclength as a parameter is that it naturally provides a way to follow the boundary, 
along which we can then place points. 
\begin{figure}
    \label{fig:boundaryCurve:t_parameter}
    \centering
    \includegraphics[width=0.6\linewidth]{pics/smoothing/t_parameter_data.pdf}
\caption{The parameter data.}
\end{figure}
Now we have data $(\tilde t_j, \tilde p_j, \tilde q_j)$, which we subdivide into two groups: $(\tilde t_j, \tilde p_j)$ and $(\tilde t_j, \tilde q_j)$. 
Since $\tilde t_j$ might initially not be equidistant, we make an equidistant sequence of samples $t_j$ and then 
use a piecewise linear interpolation operator $\pi$ to resample both data groups onto an equidistant grid:
\begin{equation}
    p = \pi \tilde p,\quad q = \pi \tilde q.
\end{equation}
\begin{figure}
    \label{fig:boundaryCurve:p_and_q_data_smooth}
    \centering
    \includegraphics[width=0.49\linewidth]{pics/smoothing/p_coordinate.pdf}
    \includegraphics[width=0.49\linewidth]{pics/smoothing/q_coordinate.pdf}
\caption{Markers correspond to the data, the green and the orange line to the final result, a smooth periodic curve approximating data in the least-squares sense.}
\end{figure}

The goal is to find a coordinate pair which smoothly depends on $t$. 
Since $t= t(p,q)$ is by definition a monotonically increasing function, we can 
look for its inverse function by approximating two 1D functions $p=p(t)$ and $q=q(t)$ 
using the parameter data computed in 
\eqref{eq:boundaryCurve:parameter}. We use \eqref{eq:rbffd:evaluation} in 1D to express the two unknown functions:
\begin{equation}
\begin{aligned}
    \label{eq:boundaryCurve:ansatz}
p(y) &=& E(y,X) c_p \\
q(y) &=& E(y,X) c_q 
\end{aligned}
\end{equation}
where $c_p$ and $c_q$ are unknown coefficients, computed such that $p(t)$ and $q(t)$ approximate the data 
$p(t_j)$ and $q(t_j)$ in the least-squares sense. We write that 
$y = Y = [t_1, t_2, ..., t_M]$ and then form two rectangular systems:
\begin{equation}
\begin{aligned}
    \label{eq:boundaryCurve:system_tmp}
    p(Y) &=& E(Y,X) c_p \\
    q(Y) &=& E(Y,X) c_q 
\end{aligned}
\end{equation}
where $X$ is a set of $N = \lceil \frac{M}{2} \rceil$ 
equidistant interpolation points $X$ in 1D.
The evaluation weights in matrix $E$ are computed using a fifth order polyharmonic spline basis, where we also append a fifth 
order polynomial degree. 
The solution of the first rectangular system from 
\eqref{eq:boundaryCurve:system_tmp} is: $c_p = E^+\, p(T),$
where $E^+ = (E^T E)^{-1} E^T$ is a pseudoinverse of $E$. 
A set of $p$- coordinates can then be evaluated using $c_p$ plugged into 
\ref{eq:boundaryCurve:system_tmp}, where we now instead of using $Y$, 
use an equidistantly sampled parameter t denoted as $T_e$:
$$p(T_e) = E(T_e, X)\, c_p = E(T_e, X) E^+(Y, X).$$
This is a temporary least-squares approximation of $p(t)$, since it is not periodic yet, i.e. 
$p(t_0) \neq p(t_{\text{end}})$.
In order to enforce the periodic conditions, we force the function values and 
all of the derivatives up to 
degree $n$ to have the same values in the first and the last parameter point. 
We first obtain all derivatives up to $n$ in point $t_1$ by applying $D^\mathcal{L}_n(t_1,X)$ from \eqref{eq:rbffd:differentiation} to $c_p$. 
Then we recompute the coefficients $c_p$ to meet the periodic conditions 
by reformulating 
\eqref{eq:boundaryCurve:system_tmp} such that:
\begin{equation}
    \label{eq:boundaryCurve:system}
\begin{pmatrix}
2 E^T E & B^T \\
B & 0
\end{pmatrix}
\begin{pmatrix}
    c_p^{(p)} \\
\lambda
\end{pmatrix}  
=  
\begin{pmatrix}
    2 E^T p(T) \\
    b
\end{pmatrix}.   
\end{equation}
Here $c_p^{(p)}$ are the coefficients corresponding to a periodic representation of $p(t)$, 
$\lambda$ a set of Lagrange multipliers and:
\begin{equation*}
B =
\begin{pmatrix}
    E(t_1,X) \\
    D^\mathcal{L}_1(t_1,X) \\
    \vdots \\
    D^\mathcal{L}_4(t_1,X) \\    
    E(t_{\text{end}},X) \\
    D^\mathcal{L}_1(t_{\text{end}},X) \\
    \vdots \\
    D^\mathcal{L}_4(t_{\text{end}},X) \\        
\end{pmatrix}
\quad
b =
\begin{pmatrix}
    E(t_1,X) c_p \\
    D^\mathcal{L}_1(t_1,X) c_p \\
    \vdots \\
    D^\mathcal{L}_4(t_1,X) c_p \\
    E(t_1,X) c_p \\
    D^\mathcal{L}_1(t_1,X) c_p \\
    \vdots \\
    D^\mathcal{L}_4(t_1,X) c_p \\           
\end{pmatrix}.
\end{equation*}
After the system \eqref{eq:boundaryCurve:system} is solved for $c_p^{(p)}$ and $\lambda$, we disregard $\lambda$ 
and use $c_p^{(p)}$ to compute a periodic representation of $p(t)$ sampled in $T_e$: 
$$p^{(p)}(T_e) = E(T_e, X)\, c_p^{(p)}.$$
Exactly the same procedure is repeated to obtain a periodic representation $q(t)$, the only difference is that we start with the different data 
and then first compute $c_q$ and then $c_q^{(p)}$, which we then use to compute a periodic representation of $q(t)$ sampled in $T_e$:
$$q^{(p)}(T_e) = E(T_e, X)\, c_q^{(p)}.$$
The points over the boundary are given by:
$$Y_b = \left[p^{(p)}(T_e),\, q^{(p)}(T_e))\right].$$
The normals in the same points are based on the first derivatives of $p^{(p)}(T_e)$ and $q^{(p)}(T_e)$:
\begin{equation*}
    p_\nabla^{(p)}(T_e) = D^\nabla(T_e, X)\, c_p^{(p)} \qquad q_\nabla^{(p)}(T_e) = D^\nabla(T_e, X)\, c_q^{(p)},
\end{equation*}
where the normals at parameter points $T_e$ are given by:
$$n = \frac{\left[p_\nabla^{(p)}(T_e), q_\nabla^{(p)}(T_e)\right]}{\sqrt{\left(p_\nabla^{(p)}(T_e)\right)^2 + \left(q_\nabla^{(p)}(T_e)\right)^2}}$$

==> sections/6_smoothing_bfuncs.tex <==
\section{Smoothing of geometry and boundary data}
\label{sec:smooth}
% Arbitrary parametrization of the curve 0 to 2pi
% Identification of the two endpoints
% Data given at T_e center points given at T_c
% Interpolation of a function to get smooth rep. Which spline is used?
% Constraint for periodicity
% Leading to linear system of the form.
% What specifically do we do with the data?
If we view the two-dimensional diaphragm from the continuous perspective, the geometry can be described as a closed curve. We choose to parametrize this curve by $t\in[0,\,2\pi]$, where the starting point $t=0$ is the same as the final point $t=2\pi$. To benefit from the potential high-order convergence of the unfitted RBF-FD method, we need to approximate the boundary curve and the boundary data as functions of $t$ with enough smoothness that the convergence of the PDE problem is not adversely affected.
%
% How do we express the function and data and the points.
% N_g uniformly spaced node points and M_g data points. Lets not call this u.
% Boundary data is g and h, f is reserved. g_j\approx(g(t_j))
To avoid reduced accuracy due to boundary errors near the artificial end points of the interval, we extend the domain periodically to $t\in[-2\pi,\,4\pi]$ for the approximation.
We discretize the extended domain using the uniformly spaced node points $T=\{t_j\}_{j=1}^{N_g}$.
%, where $t_1=0$ and $t_{N_g}=2\pi$.
Given $\tilde{M}_g$ data points, we replicate these periodically to get the extended data set $(T^d,G)=\{(t^d_i,g_i)\}_{i=1}^{M_g}$, where $M_g=3\tilde{M}_g>N_g$. We use a one-dimensional RBF-FD approximation, based on a quintic PHS basis augmented with polynomials of degree $p_g=6$,
to form an overdetermined linear system for the nodal values $g(T)$
\begin{equation}
  E_g(T^d,T)g(T)=G.
\end{equation}
%
% Add periodicity constraints
%
To enforce continuity at $t=0$, we add the following equality constraints
\begin{equation}
  %  D_t^sg(t_1) - D_t^sg(t_{N_g}),\quad s=0,\ldots,p_{\max}-1,
  \frac{d^sg(0)}{dt^s} - \frac{d^sg(2\pi)}{dt^s} = 0,\quad s=0,\ldots,p_g-1,
  \label{eq:constr}
\end{equation}  
%where $p_{\max}=5$ is the largest polynomial degree used in the numerical experiments,
and solve the constrained least squares problem
\begin{equation}
    \label{eq:boundary:system}
\begin{pmatrix}
2 E_g^T E_g & B_g^T \\
B_g & 0
\end{pmatrix}
\begin{pmatrix}
    g(T) \\
\lambda
\end{pmatrix}  
=  
\begin{pmatrix}
    2 E_g^T G \\
    0
\end{pmatrix},
\end{equation}
where $B_g$ contains the $p_g$ constraints~\eqref{eq:constr} and $\lambda$ contains the corresponding Lagrange multipliers. %For the RBF-FD approximation a quintic PHS basis augmented with polynomials of degree $p=5$ is used.

% Preprocessing of the boundary data.
% Compute the arclength using the Euclidean distance between the data points and% scale the total length to 2pi
% Downsample.
% Can place points uniformly
To find the smooth boundary curve from the initial vertex data $\tilde{x}_i^d$, $i=1,\ldots,\tilde{M}_g$, we first scale the data such that $x_i^d=(p_i,q_i)=s_\Omega\tilde{x}_i^d$, $i=1,\ldots,\tilde{M}_g$, where $s_\Omega=156.92^{-1}$\text{mm}$^{-1}$. 
The scaling was chosen such that all data points fall within $[-1,\,1]^2$. Then we compute an approximate arclength parametrization using the Euclidean distance between the scaled vertices, such that $t_i^d=2\pi\sum_{j=1}^{i-1}\|x_{j+1}^d-x_{j}^d\|/\sum_{j=1}^{\tilde{M}_g}\|x_{j+1}^d-x_j^d\|$, where $x_{\tilde{M}_g+1}^d=x_1^d$. Then we replicate the data over the extended domain.
%The total arclength is scaled down to $2\pi$ and each vertex is associated with a value of $t$.
%The number of node points is set to \textcolor{red}{$N_g=X$} and the dense vertex data is interpolated onto a smaller set of $M_g=105$ evaluation points.
Finally, system~\eqref{eq:boundary:system} is solved for each coordinate function $p(t)$ and $q(t)$. The resulting boundary curve is shown in Figure~\ref{fig:boundary} and the individual coordinate functions are shown in Figure~\ref{fig:p_and_q}. Since the curve parametrization here is in the clockwise direction, 
the outward normals are computed as $n(t) = (-q'(t),p'(t))/\|(-q'(t),p'(t))\|$. 
%\begin{equation}
%    \label{eq:experiments:diaphragm_scaling}
%\bar y = y\, s_\Omega \approx y\, \frac{1}{156.92\, mm},
%\end{equation}
%where the scaling $s_\Omega$ was chosen according to the largest coordinate of a point $y \in \Omega$.
%
% It should work well to take any subset of the data instead of interpolating.
%
% \tilde{M_g} = 177, n=28 
\begin{figure}[h!]
    \centering
    \hspace*{-1mm}\includegraphics[width=0.51\linewidth]{pics/smoothing/diaphragm_fit.pdf} \\
    \includegraphics[width=0.65\linewidth]{pics/smoothing/diaphragm_points.pdf}
    \caption{The smoothed boundary geometry curve (solid line) is shown in both subfigures. 
    The curve was computed using $N_g=133$ node points, $M_g=177\cdot 3=531$ data points, and stencil size $n=28$. 
    The markers show the $\tilde{M}_g=177$ vertex data points (top) and uniform evaluation points (bottom). 
    The normals computed from the approximation, as well as the values of the parameter $t$ along the curve, are also shown in the bottom subfigure.
%      and periodic boundary of the diaphragm Left: markers correspond to the input data points, the displayed red curve is the final smooth and periodic boundary of the diaphragm. Right: The displayed red curve 
%is the final smooth and periodic boundary of the diaphragm and the markers placed on top represent a nearly equispaced point set over the boundary of the diaphragm. The arrows 
      %display a smooth distribution of the outward normals.
    }
    \label{fig:boundary}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.49\linewidth]{pics/smoothing/p_coordinate.pdf}
    \includegraphics[width=0.49\linewidth]{pics/smoothing/q_coordinate.pdf}
    \caption{The two smoothed coordinate functions approximating the geometry. The function $p(t)$ (left) corresponds to the horizontal coordinate and $q(t)$ (right) corresponds to the vertical coordinate. The markers show the initial data locations.} %Markers correspond to the data, the green and the orange line to the final result, a smooth periodic curve approximating data in the least-squares sense.
    \label{fig:p_and_q}
\end{figure}

% I am skipping figure 6. 105 points

% Aditional things to say: How much oversampling. Or does that go into the specific section perhaps. N and M to describe the sets. N_b and M_b perhaps.
% Specific values of N and M
% Data is not so accurate. Which smoothness order we use, quintic enough for p=5. Expected convergence. see where it is mentioned.
% quintic + p=5
% We can add the equation for the normals.
% Stencil size

% Which figures are relevant here?
% Figure 7 is the geometry.
% Figure 8, I am not sure about. Does not go from zero to 2pi.
% Figure 10, yes
% Figure 11, possibly with that, but it is also good to have close to the problem.
% Figures 17, and 18. The down side is that it is far from the data. However, this is just before the benchmarks.

For the boundary data functions $g$ and $h$ in~\eqref{eq:model:naviercauchy}, we manufacture data to mimic 
the expected physiological behaviour shown in Figure~\ref{fig:smoothing:bcPosition}. A few data points are placed in the regions where we have some 
information (regions 1, 3, 5, 7, and 9 in Figure~\ref{fig:smoothing:bcPosition}), and then the rest of the data is generated through linear interpolation. 
This results in gradual transitions in the regions where we lack information. The data points and the resulting curves are shown in 
Figures~\ref{fig:experiments:Dirichlet:Diaphragm:boundary_data} and~\ref{fig:experiments:Diaphragm:Robin:boundary_data}.




% Enforce data in some regions to mimic the behaviour then create a smooth linear transition.
% Prescribe a desired behaviour

% The figure with Dirichlet data \label{fig:experiments:Dirichlet:Diaphragm:boundary_data}

% The deformed geometry \label{fig:experiments:Dirichlet:Diaphragm:deformed}
% Perhpas it is not needed to refer to this.

% The Neumann case \label{fig:experiments:Diaphragm:Robin:boundary_data}
% Why is there traction data u_1 and u_2? The force has a direction?

% specified Data and resulting curves


==> sections/7_experiments_benchmark_Dirichlet.tex <==
\section{\victor{Benchmark I: Deformation of the diaphragm using the smoothed Dirichlet boundary conditions}}
\label{sec:experiments:dirichlet}
In this section we solve the discretized linear elasticity equations \eqref{eq:method:DandF}. 
We are interested in whether the problem with smoothed Dirichlet 
boundary condition 
leads to a high-order convergence. A point of interest is also whether the resulting deformation is 
physiologically sensible, and whether the Von Mises stress is distributed as expected.

The boundary condition that we use is purely Dirichlet, which means
that we set the Robin coefficients in \eqref{eq:model:PDE} 
to $\kappa_0(y) = 1$ and $\kappa_1(y)=0$. Then the only boundary data functions present in the system 
\eqref{eq:method:DandF} are $g_1(y)$ and $g_2(y)$, which correspond 
to the imposition of displacements in the horizontal and vertical direction, respectively.

\subsection{The imposition of boundary displacements}
%
%
%We subdivide the boundary of the diaphragm into disjoint regions (see Figure~\ref{fig:smoothing:bcPosition}), 
%over which we enforce different displacements.
The displacements have been synthesized to reproduce the physiological behavior described in Section 
\ref{section:diabehavior}. Particularly, the translation of the horizontal part of the diaphragm (region 5) has been defined as a constant vertical displacement 
in the downward direction and the thickening of the appositional zone (regions 3 and 5) is also prescribed as a constant. 
As described in Section~\ref{sec:smooth}, we place a few data points based on this information, and then the rest of the data is 
generated by linear interpolation. From a physiological perspective all displacements should be smooth. 
We generate a smooth function by solving the constrained least squares problem~\eqref{eq:boundary:system}. 
%
%\begin{figure}[h!]
%\centering
%\includegraphics[width=0.85\linewidth]{pics/smoothing/BCs.png}
%\caption{Benchmark I: Boundary conditions: displacements on 9 area of the diaphragm. Red areas correspond to the real physiological behaviors and the green areas are transition zones.}\label{fig:BCs}
%\label{fig:smoothing:bcPosition}
%\end{figure}
%
%At first, the displacements are discontinuous. To make the displacements smooth
%we fit a smooth curve through the discontinuities 
%using the smoothing procedure described in 
%Section \ref{sec:smoothing_BCdata}.
The results are shown in Figure~\ref{fig:experiments:Dirichlet:Diaphragm:boundary_data}.
Imposing smooth boundary data makes it possible to obtain high-order convergence and provides a solution that is physically relevant. 
%
\begin{figure}[htb!]
    \centering
    \begin{tabular}{@{}cc@{}}
        \hspace{1.3cm}\textbf{Displacement $\mathbf{\tilde u_1}$} & \hspace{1.3cm}\textbf{Displacement $\mathbf{\tilde u_2}$} \\
        \includegraphics[height=0.22\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Data/bndry_data_Dirichlet_u1.pdf} & 
        \raisebox{0.005\linewidth}{\includegraphics[height=0.22\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Data/bndry_data_Dirichlet_u2.pdf}}
    \end{tabular}
    \caption{Benchmark I: The displacement in the horizontal direction (left) and the vertical direction (right) as a 
    function of the boundary parametrization $t$ (see Figure~\ref{fig:boundary}, right image, for an illustration of $t$ in relation to the boundary). The markers show the initially placed data points, which are then linearly interpolated into $\tilde{M}_g=80$ data points. For the approximation, $N_g=120$ node points and stencil size $n=28$ were used. 
    The dashed lines show the location of the end points of the diaphragm (regions 2 and 8 in Figure~\ref{fig:smoothing:bcPosition}).}
    \label{fig:experiments:Dirichlet:Diaphragm:boundary_data}
\end{figure}
In Figure~\ref{fig:experiments:Dirichlet:Diaphragm:deformed} we display the boundary of the diaphragm before and after 
application of the displacements from Figure~\ref{fig:experiments:Dirichlet:Diaphragm:boundary_data}.
\begin{figure}[htb!]
    \centering
    \includegraphics[width=0.6\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Solution/diaphragm_deformed.pdf}
    \caption{Benchmark I: The diaphragm in its non-deformed state (dashed line) and after displacement of the boundary (solid line).}
    \label{fig:experiments:Dirichlet:Diaphragm:deformed}
\end{figure}
%\subsection{Convergence under node refinement to FEM as reference (Pierre)}
%\input{sections/fem1.tex}
\subsection{Solution of Benchmark I}
The solution is given in Figure~\ref{fig:experiments:Dirichlet:Diaphragm:solution}, 
where we display the spatial distribution of the displacements and the Von Mises stress. 
Looking at the $\tilde u_1$ distribution in the figure, we can observe thickening of the diaphragm 
in regions 2, 3, 7 and 8 according to the labels from Figure~\ref{fig:smoothing:bcPosition}. 
Next, the distribution of $\tilde u_2$ indicates that translation is largest in regions 4, 5 and 6. 
The Von Mises stress is largest at the interfaces between regions 2, 3 and regions 7, 8. \elisabeth{This makes sense, since the change in the thickness is largest in these regions}. 
We conclude that the behavior roughly follows the 
physiological cues described in Section~\ref{section:diabehavior}.
%\begin{figure}[h!]
%    \centering    
%    \begin{tabular}{c}
%    \textbf{Displacement $\tilde u_1$} \\
%    \includegraphics[width=0.85\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Solution/solution_numRef_abs_u1.png} \\
%    \textbf{Displacement $\tilde u_2$} \\
%    \includegraphics[width=0.85\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Solution/solution_numRef_abs_u2.png} \\
%    \textbf{Von Mises stress} \\
%    \includegraphics[width=0.85\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Solution/solution_numRef_abs_vonMises.png}
%    \end{tabular}
%    \caption{Benchmark I:  Three computed solution quantities over a diaphragm. This solution was obtained using the unfitted RBF-FD discretization with internodal distance $h=0.004$, 
%    an oversampling parameter $q=5$ and an appended polynomial basis of degree $5$. \victor{The conventional displacement and stress units are normalized using the scaling $s_{\Omega} = 0.15692^{-1}\, \text{m}^{-1} = 156.92^{-1}\, \text{mm}^{-1}$, provided in Section \ref{sec:smooth}.}}
%    \label{fig:experiments:Dirichlet:Diaphragm:solution}
%\end{figure}
\begin{figure}[h!]
    \centering    
    \begin{tabular}{c}
    \textbf{Displacement $\tilde u_1$} \\
    \includegraphics[width=0.65\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Solution/solution_numRef_abs_u1.png} \\
    \textbf{Displacement $\tilde u_2$} \\
    \includegraphics[width=0.65\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Solution/solution_numRef_abs_u2.png} \\
    \textbf{Von Mises stress} \\
    \includegraphics[width=0.65\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Solution/solution_numRef_abs_vonMises.png}
    \end{tabular}
    \caption{Benchmark I:  The computed displacements and the corresponding von Mises stress over the diaphragm. This solution was obtained using the unfitted RBF-FD discretization with internodal distance $h=0.004$, 
    oversampling parameter $q=5$, and an appended polynomial basis of degree $p=5$. \victor{Due to the scaling applied to the geometry (see Section~\ref{sec:smooth}), the displayed results for displacement and stress 
    should be multiplied with $s_{\Omega}^{-1} = 0.15692$ m to recover the results corresponding to the unscaled problem.}}
    \label{fig:experiments:Dirichlet:Diaphragm:solution}
\end{figure}

\subsection{Convergence under node refinement}
While the solution is roughly what we expect from a physiological perspective, we are yet to understand whether 
the simulation gives a correct answer from a numerical perspective. 
We investigate the convergence of the numerical solution under node refinement using several different 
polynomial degrees in the stencil-based approximation.
Since we do not know what the true solution is, we measure convergence of the numerical solution $\tilde u(Y)$ towards a numerical reference 
solution $\tilde u_*(Y_*)$, where \elisabeth{the node set is highly refined}. We choose two numerical references: 
(i) computed using the unfitted RBF-FD-LS method with internodal distance $h=0.002$, leading to $N=43\,841$ and polynomial degree $p=5$,  
(ii) computed using the Galerkin finite element method with 
linear elements and $236\,414$ degrees of freedom (corresponding to $h = 0.00085$), using the GetDP solver \cite{getdp-siam2008}. 
Every numerical solution $\tilde u$ that we obtain is interpolated, \victor{consistent with the approximation order,} to the point set 
of the reference solution $Y_*$, where we then compute the approximation error:
\begin{equation}
    \label{eq:dirichlet:error}
\| e \|_{\ell_2} = \frac{\|\tilde u(Y_*) - \tilde u_*(Y_*)\|_2}{\|\tilde u_*(Y_*)\|_2}.
\end{equation}
\begin{figure}[h!]
    \centering
    \begin{tabular}{ccc}
        \hspace{0.9cm}\textbf{Displacement } $\mathbf{\tilde u_1}$ & \hspace{0.9cm}\textbf{Displacement } $\mathbf{\tilde u_2}$ & \hspace{0.9cm}\textbf{Von Mises} \\
        \includegraphics[width=0.315\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/Self/Error_u1.pdf} &  
        \includegraphics[width=0.315\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/Self/Error_u2.pdf} &  
        \includegraphics[width=0.315\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/Self/Error_vonMises.pdf}  
    \end{tabular}        
    % \begin{tabular}{cc}
    % \hspace{1cm}$p=2$ & \hspace{1cm}$p=3$ \\
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/Self/Error_polydeg=2.pdf}  &  
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/Self/Error_polydeg=3.pdf} \\
    % \hspace{1cm}$p=4$ & \hspace{1cm}$p=5$ \\
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/Self/Error_polydeg=4.pdf}  &  
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/Self/Error_polydeg=5.pdf}
    % \end{tabular}
    \caption{Benchmark I: Convergence of the displacements $\tilde u_1$ and $\tilde u_2$ and the Von Mises stress for different polynomial degrees $p$, 
    against a highly resolved numerical solution computed using the unfitted RBF-FD-LS method, \victor{with $h=0.002$ and $p=5$}.}
    \label{fig:experiments:Dirichlet:Diaphragm:convergence_selfRef}
\end{figure}
Table~\ref{fig:experiments:Dirichlet:Diaphragm:h_to_N_table} shows the relation between the 
internodal distance $h$, computed according to \eqref{eq:method:h_and_hy}, and the number of degrees of freedom $N$ for the considered problem sizes. 
\begin{table}[h!]
    \centering
    \caption{Benchmark I and II: The relation between the inverse internodal distance $1/h$ and (i) the internodal distance $h$ and (ii) the number of interpolation points $N$ used for discretizing the PDE problem \eqref{eq:model:PDE}.}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
      %\multicolumn{9}{c}{\textbf{Relation between $\mathbf{1/h}$, $\mathbf{h}$ and $\mathbf{N}$} \vspace{1.5mm}} \\
      \hline
        $\mathbf{1/h}$ & 25 & 50 & 100 & 125 & 166.67 & 200 & 250 & 500 \\ \hline
        $\mathbf{h}$ &  0.04 & 0.02 & 0.01 & 0.008 & 0.006 & 0.005 & 0.004 & 0.002 \\ %\hline
        $\mathbf{N}$ & 337 & 853 & 2500 & 3617 & 5904  & 8126 & 12129 & 43841 \\
        \hline
    \end{tabular}        

    \label{fig:experiments:Dirichlet:Diaphragm:h_to_N_table}
\end{table}

The results when the unfitted RBF-FD method is used as a reference are displayed in Figure~\ref{fig:experiments:Dirichlet:Diaphragm:convergence_selfRef}. 
We observe that the error is small for all polynomial degrees. \elisabeth{The convergence rate increases as $p$ is increased.} 
For all $p$ the convergence rates of the displacements are close to $p-1$. 
The convergence rate of the Von Mises stress is larger than $p-2$ for every $p$. 
Stress is computed using the first derivatives of the displacements, which (in theory) lowers the 
convergence rate with one \elisabeth{order}.

The results when the finite element method is used as a reference are given in Figure~\ref{fig:experiments:Dirichlet:Diaphragm:convergence_femRef}. 
The convergence plots for the displacement are very similar to the results in Figure~\ref{fig:experiments:Dirichlet:Diaphragm:convergence_selfRef}.
The convergence rate of the stress for $p=5$ is \elisabeth{lower} compared with the self-reference test provided in Figure~\ref{fig:experiments:Dirichlet:Diaphragm:convergence_selfRef}. 
Furthermore, when $p=5$, the convergence seems to be stalling at the last point of observation. 
Our speculative reasoning is that the derivatives in the finite element space 
do not approximate the stresses well enough there. 
This implies that the FEM mesh is too coarse to match the accuracy of the unfitted RBF-FD method for derivative approximation, 
when the polynomial degree is as high as $p=5$, for the range of $h$ used here.
\begin{figure}[h!]
    \centering
    \begin{tabular}{ccc}
        \hspace{0.9cm}\textbf{Displacement }$\mathbf{\tilde u_1}$ & \hspace{0.9cm}\textbf{Displacement }$\mathbf{\tilde u_2}$ & \hspace{0.9cm}\textbf{Von Mises} \\
        \includegraphics[width=0.315\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/FEM/Error_u1.pdf} &  
        \includegraphics[width=0.315\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/FEM/Error_u2.pdf} &  
        \includegraphics[width=0.315\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/FEM/Error_vonMises.pdf}  
    \end{tabular}    
    % \begin{tabular}{cc}
    % \hspace{1cm}$p=2$ & \hspace{1cm}$p=3$ \\
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/FEM/Error_polydeg=2.pdf}  &  
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/FEM/Error_polydeg=3.pdf} \\
    % \hspace{1cm}$p=4$ & \hspace{1cm}$p=5$ \\
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/FEM/Error_polydeg=4.pdf}  &  
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/FEM/Error_polydeg=5.pdf}
    % \end{tabular}
    \caption{Benchmark I: Convergence of the displacements $\tilde u_1$ and $\tilde u_2$ and the Von Mises stress for different polynomial degrees $p$, 
    against a highly resolved numerical solution computed using FEM \victor{(the GetDP solver \cite{getdp-siam2008}) with linear elements and $236\,414$ degrees of freedom (corresponding to $h = 0.00085$).}}
    \label{fig:experiments:Dirichlet:Diaphragm:convergence_femRef}
\end{figure}

The spatial distribution of the error when using the self-reference solution and the finite element reference solution 
is shown in Figure 
\ref{fig:experiments:Dirichlet:Diaphragm:error_spatial_selfRef} and Figure~\ref{fig:experiments:Dirichlet:Diaphragm:error_spatial_femRef}, 
respectively. The numerical solution was computed using $h=0.004$, $q=5$, $p=5$.
\elisabeth{For all solution fields and both references we can observe that the error is larger in the regions with larger Von Mises stress. In addition, the error also tends to be larger in the regions where 
the boundary curve is concave. This implies that our problem could benefit from adaptive 
node refinement, which we are planning to use in our future work.}

\begin{figure}[h!]
    \centering
    \begin{tabular}{cc}
    \textbf{Displacement $\tilde u_1$} & \textbf{Displacement $\tilde u_2$} \\
    \includegraphics[width=0.49\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Error_distribution/err_numRef_abs_u1.png} &
    \includegraphics[width=0.49\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Error_distribution/err_numRef_abs_u2.png} \\
    \multicolumn{2}{c}{\textbf{Von Mises stress}} \\
    \multicolumn{2}{c}{\includegraphics[width=0.6\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Error_distribution/err_numRef_abs_vonMises.png}}
    \end{tabular}
    \caption{Benchmark I: Error distribution in logarithmic scale for $h=0.006$ and $p=5$ when a fine unfitted RBF-FD-LS solution ($h=0.002$, $p=5$) 
    is taken as reference for computing the error.}
    \label{fig:experiments:Dirichlet:Diaphragm:error_spatial_selfRef}
\end{figure}

\begin{figure}[h!]
    \centering
    \begin{tabular}{cc}
    \textbf{Displacement $\tilde u_1$} & \textbf{Displacement $\tilde u_2$} \\
    \includegraphics[width=0.49\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Error_distribution/err_u1_rbfVsfem.png} &
    \includegraphics[width=0.49\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Error_distribution/err_u2_rbfVsfem.png} \\
    \multicolumn{2}{c}{\textbf{Von Mises stress}} \\
    \multicolumn{2}{c}{\includegraphics[width=0.6\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Error_distribution/err_vonMises_rbfVsfem.png}}
    \end{tabular}
    \caption{Benchmark I: Error distribution in logarithmic scale for $h=0.006$ and $p=5$ when a fine unfitted RBF-FD-LS solution ($h=0.002$, $p=5$) 
    is taken as reference for computing the error.}
    \label{fig:experiments:Dirichlet:Diaphragm:error_spatial_femRef}
\end{figure}


==> sections/7_smoothing.tex <==
\section{Smoothing of the boundary condition data}
\label{sec:smoothing_BCdata}
We are given an input vector $\tilde f(T_e)$ with discontinuous data sampled over the parameter points $T_e$.

First, we reduce the data such that only a few points ($3$ to $7$ in our experiments) per a continuous subinterval are kept, discarding 
the points on the edges of those subintervals. This results into obtaining two reduced vectors, $\tilde f_r$ and $T_r$. 
Then we use a piecewise 
linear interpolation onto the set of points $T_e$:
$$\bar f(T_e) = \pi \tilde f_r(T_r).$$
Now we have the data that is continuous but not smooth, an example is given in the first plot of Figure \ref{fig:smoothing:data_and_final}.

\begin{figure}[h!]
    \label{fig:smoothing:data_and_final}
    \centering
    \includegraphics[width=0.49\linewidth]{pics/smoothing/smoothing_example_data.pdf}
    \includegraphics[width=0.49\linewidth]{pics/smoothing/smoothing_example_final.pdf}
    \caption{Row 1: The blue curve shows the original discontinuous data, the black markers the reduced data over the blue curve 
    and the black curve the linear interpolation between the black markers. Row 2: The red curve displays the final smoothed and periodic curve.}
\end{figure}


The next steps closely follow the ones from Section \ref{sec:smoothDiaphragmBoundaryCurve}, where we make a smooth representation of the data, 
and in addition make it periodic at the ends of the interval, both in function values and its derivatives up to degree $n$.
We look for the unknown coefficents $c_f$ from a relation:
$$E(T_e,X)\, c_f = \bar f(T_e),$$
where we choose the point set $X$ to be of size $N=\lceil \frac{M}{2} \rceil$. 
The coefficients are given by $c_f = E^+(T_e,X)\, \bar f(T_e)$, and an evaluation of a smooth curve $f$ sampled in $T_e$ is given by:
$$f(T_e) = E(T_e,X)\, E^+(T_e,X)\, \bar f(T_e).$$
This is only a temporary least-squares approximation of $f$, since we have not made it periodic yet, i.e. 
$f(t_0) \neq f(t_{\text{end}})$.
In order to enforce the periodic conditions, we force the function values and 
all of the derivatives up to 
degree $n$ to have the same values in the first and the last parameter point. 
We first obtain all derivatives up to $n$ in a point 
$t_1$ by applying $D^\mathcal{L}_n(t_1,X)$ to $c_f$. 
Then we recompute the coefficients $c_f$ to meet the periodic conditions 
by solving a system:
\begin{equation}
\begin{pmatrix}
2 E^T E & B \\
B^T & 0
\end{pmatrix}
\begin{pmatrix}
    c_f^{(p)} \\
\lambda
\end{pmatrix}  
=  
\begin{pmatrix}
    2 E^T f(T_e) \\
    b
\end{pmatrix}.   
\end{equation}
Here $c_f^{(p)}$ are the coefficients corresponding to a periodic representation of $f$, 
$\lambda$ a set of lagrange multipliers and:
\begin{equation*}
B =
\begin{pmatrix}
    E(t_1,X) \\
    D^\mathcal{L}_1(t_1,X) \\
    \vdots \\
    D^\mathcal{L}_4(t_1,X) \\    
    E(t_{\text{end}},X) \\
    D^\mathcal{L}_1(t_{\text{end}},X) \\
    \vdots \\
    D^\mathcal{L}_4(t_{\text{end}},X) \\        
\end{pmatrix}
\quad
b =
\begin{pmatrix}
    E(t_1,X) c_p \\
    D^\mathcal{L}_1(t_1,X) c_p \\
    \vdots \\
    D^\mathcal{L}_4(t_1,X) c_p \\
    E(t_1,X) c_p \\
    D^\mathcal{L}_1(t_1,X) c_p \\
    \vdots \\
    D^\mathcal{L}_4(t_1,X) c_p \\           
\end{pmatrix}
\end{equation*}
After the system is solved for $c_f^{(p)}$ and $\lambda$, we disregard $\lambda$ 
and use $c_f^{(p)}$ to compute a periodic representation of $f(t)$ sampled in $T_e$: 
$$f^{(p)}(T_e) = E(T_e, X)\, c_f^{(p)}.$$ An example of a final smooth and periodic curve is displayed in 
Figure \ref{fig:smoothing:data_and_final}.

==> sections/8_experiments_inwardCorners.tex <==
\section{An investigation of high-order convergence using custom PDE data}

\begin{itemize}
    \item This is an experiment which indicates the relation of high-order convergence to the shape of domain.
    \item A circle has no inward ''smooth corners''. Convergence rate is pretty much what it should be.
    \item A star has plenty gentle inward ''smooth corners''. Convergence rate stalls when as the polynomial degree is increased.
    \item A look at the absolute errors reveals artefacts that start to appear at the smooth ''inward corners'' in the star geometry case.
    \item The diaphragm has smooth ''inward corners''. According to results above, not observing optimal convergence rates is fine.
\end{itemize}

Theta is a parameter over the boundary. We solve:
\begin{eqnarray*}
\Delta u(x,y) &=& \cos(2\pi x y), \text{ on } \Omega \\
u(\theta) &=& \sin(\theta), \text{ on } \partial\Omega
\end{eqnarray*}
Results are in Figure \ref{fig:experiments:inwardcorners:solution_and_errors_href} and Figure \ref{fig:experiments:inwardcorners:error_spatialdistributions}.

\begin{figure}
    \centering
    \includegraphics[width=0.48\linewidth]{pics/experiments_highorder_customData/Circle/Solution_h=0_008_p=6.png}
    \includegraphics[width=0.39\linewidth]{pics/experiments_highorder_customData/Circle/Error_numericalRef_manyPolydegs.pdf} \\    
    \includegraphics[width=0.48\linewidth]{pics/experiments_highorder_customData/StarShaped/Solution_h=0_008_p=6.png}
    \includegraphics[width=0.39\linewidth]{pics/experiments_highorder_customData/StarShaped/Error_numericalRef_manyPolydegs.pdf}
    \caption{Left: solution of the Poisson equation with custom right-hand-side data. Right: relative error computed as a function of the internodal distance $h$ for different choices of the polynomial degree $p$ used to construct the stencil approximation. Here the reference solution is taken to be a fine numerical solution at $h=0.008$ ($1/h=125$) and $p=6$.}
    \label{fig:experiments:inwardcorners:solution_and_errors_href}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/Circle/error_polydeg=2.png}
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/Circle/error_polydeg=3.png}
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/Circle/error_polydeg=4.png}    
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/Circle/error_polydeg=5.png}    
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/Circle/error_polydeg=6.png} \\        
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/StarShaped/error_polydeg=2.png}
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/StarShaped/error_polydeg=3.png}
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/StarShaped/error_polydeg=4.png}    
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/StarShaped/error_polydeg=5.png}
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/StarShaped/error_polydeg=6.png} \\

    \caption{Spatial distributions of the error in the logarithmic scale. 
    The three distributions correspond to the three polynomial degrees ($p=2$, $p=4$, $p=6$) used to construct the stencil approximations.
    The reference solution is taken to be a numerical solution at the internodal distance $h=0.008$ and $p=6$, while the approximate solution is computed at $h=0.02$.}
    \label{fig:experiments:inwardcorners:error_spatialdistributions}    
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/Circle/error_polydeg=2_log10.png}
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/Circle/error_polydeg=3_log10.png}
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/Circle/error_polydeg=4_log10.png}    
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/Circle/error_polydeg=5_log10.png}    
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/Circle/error_polydeg=6_log10.png} \\        
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/StarShaped/error_polydeg=2_log10.png}
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/StarShaped/error_polydeg=3_log10.png}
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/StarShaped/error_polydeg=4_log10.png}    
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/StarShaped/error_polydeg=5_log10.png}
    \includegraphics[width=0.19\linewidth]{pics/experiments_highorder_customData/StarShaped/error_polydeg=6_log10.png} \\

    \caption{Spatial distributions of the error in the logarithmic scale. 
    The three distributions correspond to the three polynomial degrees ($p=2$, $p=4$, $p=6$) used to construct the stencil approximations.
    The reference solution is taken to be a numerical solution at the internodal distance $h=0.008$ and $p=6$, while the approximate solution is computed at $h=0.02$.}
    \label{fig:experiments:inwardcorners:error_spatialdistributions_log10}    
\end{figure}

==> sections/9_experiments_benchmark_Dirichlet_old_or_what.tex <==
\section{Benchmark I: Deformation of the diaphragm using the smoothed Dirichlet boundary conditions}
\label{sec:experiments:dirichlet}
In this section we solve the discretizred linear elasticity equations \eqref{eq:method:DandF}. 
We are interested in whether the problem with smoothed Dirichlet 
boundary condition 
leads to a high-order convergence. Our point of interest is also whether the resulting deformation is 
physiologically sensible, and whether the Von Mises stress is distributed as expected.

The boundary condition that we use is of a purely Dirichlet type, which means
that we set the Robin coefficients $\kappa_0$ and $\kappa_1$ in \eqref{eq:method:Robincoeff} 
to $\kappa_0(y) = 1$ and $\kappa_1(y)=0$. Then the only boundary data functions present in the system 
\eqref{eq:method:DandF} are $g_1(y)$ and $g_2(y)$, which correspond 
to the imposition of displacements into horizontal and vertical directions respectively.

\subsection{The imposition of boundary displacements}

We subdivide the boundary of the diaphragm into disjoint regions (see Figure \ref{fig:smoothing:bcPosition}), 
over which we enforce different displacements.
The displacements have been synthesized to reproduce the physiological behavior described in Section 
\ref{section:diabehavior}. Particularly, the translation motion of the tendon has been defined by a constant displacement 
in the superior to inferior direction ($x$ direction) and the thickening of the appositional zone is also done in the lateral direction ($y$ direction)
in the same way. 

\begin{figure}[h!]
\centering
\includegraphics[width=0.85\linewidth]{pics/smoothing/BCs.png}
\caption{Benchmark I: Boundary conditions: displacements on 9 area of the diaphragm. Red areas correspond to the real physiological behaviors and the green areas are transition zones.}\label{fig:BCs}
\label{fig:smoothing:bcPosition}
\end{figure}

At first, the displacements are discontinuous. To make the displacements smooth
we fit a smooth curve through the discontinuities 
using the smoothing procedure described in 
Section \ref{sec:smoothing_BCdata}. Result is given in Figure \ref{fig:experiments:Dirichlet:Diaphragm:boundary_data}.
This makes it possible to obtain high-order convergence and a solution that is physically more relevant. 

\begin{figure}[h!]
    \centering
    \begin{tabular}{cc}
        \hspace{1.3cm}\textbf{Displacement $u_1$} & \hspace{0.7cm}\textbf{Displacement $u_2$} \\
        \includegraphics[width=0.49\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Data/bndry_data_Dirichlet_u1.pdf} & 
        \includegraphics[width=0.47\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Data/bndry_data_Dirichlet_u2.pdf}
    \end{tabular}
    \caption{Benchmark I: The left image shows the displacement in the horizontal direction, right image the displacement in the vertical direction, 
    both are a function of the parameter $t$ over the boundary of the diaphragm. 
    The circular data points display the imposed data, the fitted curves are smooth and periodic representations of the data.}
    \label{fig:experiments:Dirichlet:Diaphragm:boundary_data}
\end{figure}
In Figure \ref{fig:experiments:Dirichlet:Diaphragm:deformed} we display a boundary of the diaphragm before and after 
the application of displacements from Figure \ref{fig:experiments:Dirichlet:Diaphragm:boundary_data}.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Solution/diaphragm_deformed.pdf}
    \caption{Benchmark I: The diaphragm in its non-deformed state (dashed grey line) and after displacement of the boundary (full red line).}
    \label{fig:experiments:Dirichlet:Diaphragm:deformed}
\end{figure}
%\subsection{Convergence under node refinement to FEM as reference (Pierre)}
%\input{sections/fem1.tex}
\subsection{Solution of Benchmark I}
The solution is given in Figure \ref{fig:experiments:Dirichlet:Diaphragm:solution}, 
where we display the spatial distribution of the displacements and the Von Mises stress. 
Looking at the $u_1$ distribution in the figure, we can observe the thickening of the diaphragm 
in regions 2, 3, 7 and 8 according to the labels from Figure \ref{fig:smoothing:bcPosition}. 
Next, the distribution of $u_2$ indicates that translation is largest in regions 4, 5 and 6. 
The Von Mises stress is largest at the interfaces between regions 2,3 and regions 7, 8: this is sensible 
since the diaphragm is clamped below these interfaces. We conclude that the behavior roughly follows the 
physiological cues described in \ref{section:diabehavior}.
\begin{figure}[h!]
    \centering    
    \begin{tabular}{c}
    \textbf{Displacement $u_1$} \\
    \includegraphics[width=0.85\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Solution/solution_numRef_abs_u1.png} \\
    \textbf{Displacement $u_2$} \\
    \includegraphics[width=0.85\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Solution/solution_numRef_abs_u2.png} \\
    \textbf{Von Mises stress} \\
    \includegraphics[width=0.85\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Solution/solution_numRef_abs_vonMises.png}
    \end{tabular}
    \caption{Benchmark I:  Three computed solution quantities over a diaphragm. This solution was obtained using an Unfitted RBF-FD discretization with internodal distance $h=0.004$, an oversampling parameter $q=5$ and an appended 
    polynomial basis of degree $5$.}
    \label{fig:experiments:Dirichlet:Diaphragm:solution}
\end{figure}

\subsection{Convergence under node refinement}
While the solution is roughly what we expect from a physiological perspective, we are yet to understand whether 
the simulation is gives a correct answer from a numerical perspective. 
We investigate the convergence of the numerical solution under node refinement using several different 
polynomial basis degrees in the stencil based approximation.
Since we do not know what the true solution is, we measure convergence of $u_h(Y)$ towards a numerical reference 
solution $u_h^*(Y^*)$ where the node refinement is sufficiently large. We choose two numerical references: 
(i) computed using Unfitted RBF-FD using internodal distance $h=0.001$ and polynomial degree $p=5$,  
(ii) computed using the Galerkin finite element method with 
linear elements and $461138$ degrees of freedom and using GetDP solver \cite{getdp-siam2008}. Every $u_h$ that we obtain is interpolated to the point set 
of the reference solution $Y^*$, where we then compute the approximation error:
\begin{equation}
    \label{eq:dirichlet:error}
\| e \|_{\ell_2} = \frac{\|u_h(Y^*) - u_h^*(Y^*)\|_2}{\|u_h^*(Y^*)\|_2}.
\end{equation}
\begin{figure}[h!]
    \centering
    \begin{tabular}{ccc}
        \hspace{0.9cm}\textbf{Displacement } $\mathbf{u_1}$ & \hspace{0.9cm}\textbf{Displacement } $\mathbf{u_2}$ & \hspace{0.9cm}\textbf{Von Mises} \\
        \includegraphics[width=0.315\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/Self/Error_u1.pdf} &  
        \includegraphics[width=0.315\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/Self/Error_u2.pdf} &  
        \includegraphics[width=0.315\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/Self/Error_vonMises.pdf}  
    \end{tabular}        
    % \begin{tabular}{cc}
    % \hspace{1cm}$p=2$ & \hspace{1cm}$p=3$ \\
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/Self/Error_polydeg=2.pdf}  &  
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/Self/Error_polydeg=3.pdf} \\
    % \hspace{1cm}$p=4$ & \hspace{1cm}$p=5$ \\
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/Self/Error_polydeg=4.pdf}  &  
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/Self/Error_polydeg=5.pdf}
    % \end{tabular}
    \caption{Benchmark I: Convergence of displacements $u_1$ and $u_2$ and the Von Mises stress for different polynomial degrees $p$, 
    against a highly resolved numerical solution computed using Unfitted RBF-FD-LS.}
    \label{fig:experiments:Dirichlet:Diaphragm:convergence_selfRef}
\end{figure}
The results when unfitted RBF-FD is used as a reference are displayed in Figure \ref{fig:experiments:Dirichlet:Diaphragm:convergence_selfRef}. 
First, we observe that the error is small for all polynomial degrees. Second, we observe that the convergence as $h$ is decreased is 
uniform in its rate. Third, the convergence rates increase for an increase of the polynomial degree. 
For all $p$ the convergence rates of displacements are higher than $p-1$. 
The convergence rate of the Von Mises stress is larger than $p-2$ for every $p$. 
Stress is computed using the first derivatives of the displacements, which (in theory) lowers the 
convergence rate with one degree.

Results when the finite element method is used as a reference are given in Figure \ref{fig:experiments:Dirichlet:Diaphragm:convergence_femRef}. 
The numerical solution converges uniformly for all $p$. Futhermore, the convergence rates of displacements for every $p$ are at least $p-1$. 
The convergence rate of the stress is smaller compared to the self-reference test in \ref{fig:experiments:Dirichlet:Diaphragm:convergence_selfRef}. 
Furthermore, when $p=5$ the convergence seems to be stalling at the last point of observation. 
Our speculative reasoning is that the derivatives in the finite element space are only piecewise constant functions, 
which do not approximate the stresses well enough. 
This implies that the FEM mesh is too coarse for the given combination of the large 
polynomial degree ($p=5$) and the given $h$ (the last measurement point from left to right in Figure \ref{fig:experiments:Dirichlet:Diaphragm:convergence_femRef} on the 
unfitted RBF-FD side.
\begin{figure}[h!]
    \centering
    \begin{tabular}{ccc}
        \hspace{0.9cm}\textbf{Displacement }$\mathbf{u_1}$ & \hspace{0.9cm}\textbf{Displacement }$\mathbf{u_2}$ & \hspace{0.9cm}\textbf{Von Mises} \\
        \includegraphics[width=0.315\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/FEM/Error_u1.pdf} &  
        \includegraphics[width=0.315\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/FEM/Error_u2.pdf} &  
        \includegraphics[width=0.315\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/FEM/Error_vonMises.pdf}  
    \end{tabular}    
    % \begin{tabular}{cc}
    % \hspace{1cm}$p=2$ & \hspace{1cm}$p=3$ \\
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/FEM/Error_polydeg=2.pdf}  &  
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/FEM/Error_polydeg=3.pdf} \\
    % \hspace{1cm}$p=4$ & \hspace{1cm}$p=5$ \\
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/FEM/Error_polydeg=4.pdf}  &  
    % \includegraphics[width=0.29\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Convergence/FEM/Error_polydeg=5.pdf}
    % \end{tabular}
    \caption{Benchmark I: Convergence of displacements $u_1$ and $u_2$ and the Von Mises stress for different polynomial degrees $p$, 
    against a highly resolved numerical solution computed using FEM.}
    \label{fig:experiments:Dirichlet:Diaphragm:convergence_femRef}
\end{figure}

The spatial distribution of the error when using the self-reference solution and the finite element reference solution 
is shown in Figure 
\ref{fig:experiments:Dirichlet:Diaphragm:error_spatial_selfRef} and \ref{fig:experiments:Dirichlet:Diaphragm:error_spatial_femRef} 
respectively. Here the numerical solution was computed using $h=0.004$, $q=5$, $p=5$.
For all solution fields and both references we can observe that the error is significantly larger in the regions where 
the geometry of the diaphragm makes a turn. This implies that our problem would benefit from adaptive 
node refinement, which we are planning to use in our future work.

\begin{figure}[h!]
    \centering
    \begin{tabular}{cc}
    \textbf{Displacement $u_1$} & \textbf{Displacement $u_2$} \\
    \includegraphics[width=0.49\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Error_distribution/err_numRef_abs_u1.png} &
    \includegraphics[width=0.49\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Error_distribution/err_numRef_abs_u2.png} \\
    \multicolumn{2}{c}{\textbf{Von Mises stress}} \\
    \multicolumn{2}{c}{\includegraphics[width=0.6\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Error_distribution/err_numRef_abs_vonMises.png}}
    \end{tabular}
\caption{Benchmark I: Error distribution in the logarithmic scale when a fine Unfitted RBF-FD-LS solution is used as a reference solution when computing the error.}
    \label{fig:experiments:Dirichlet:Diaphragm:error_spatial_selfRef}
\end{figure}

\begin{figure}[h!]
    \centering
    \begin{tabular}{cc}
    \textbf{Displacement $u_1$} & \textbf{Displacement $u_2$} \\
    \includegraphics[width=0.49\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Error_distribution/err_u1_rbfVsfem.png} &
    \includegraphics[width=0.49\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Error_distribution/err_u2_rbfVsfem.png} \\
    \multicolumn{2}{c}{\textbf{Von Mises stress}} \\
    \multicolumn{2}{c}{\includegraphics[width=0.6\linewidth]{pics/experiments_highorder_customData/Diaphragm/Dirichlet/Error_distribution/err_vonMises_rbfVsfem.png}}
    \end{tabular}
\caption{Benchmark I: Error distribution in the logarithmic scale when a fine FEM solution is taken as a reference when computing the error.}
    \label{fig:experiments:Dirichlet:Diaphragm:error_spatial_femRef}
\end{figure}

==> sections/fem1.tex <==

We saw in \S \ref{sec:model:naviercauchy} that the mathematical description of the elasticity problem consists on solving partial differential equations. The finite element method (FEM) is a way to solve such partial differential equations in the weak form after having computed a discrete geometry. Depending on the mesh level, the solution could be very accurate. It is the reason why it is commonly used in the literature to compare and evaluate a simulation.

In order to evaluate our method, we have also implemented FEM simulations. The diaphragm contour is the same as previously (see \S {sec:dataAcquisition}). This loop of line segments was meshed with triangles using Gmsh \cite{gmsh}. Mesh edges can be seen in black on Figure~\ref{fig:femDirichelet}. Various levels of mesh accuracy has been tested. A triangle set allowing global results comparable to results obtained with significantly more elements was chosen. The mesh contains 4714 nodes and 8452 triangles and it has been computed in approximately 0.5 seconds.

GetDP solver \cite{getdp-siam2008} was used. Regions were defined such as the whole mesh is a region and each node of the contour is a region. 
The displacement to strain equation is given by the small deformation linear relationship ({\color{red}similarly to our method?}). The constitutive law is also Hooke's law. The shape function inside the triangle are of the first order and numerical Gauss integration is used. 

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics/fem/FEMDirichelet.png}
    \caption{FEM simulation with Dirichelet conditions. \textit{Red curve}: initial contour, \textit{black triangles}: deformed mesh, \textit{color scale}: Von Mises stress. ({\color{red}This figure will be changed and the colorscale will be added later})}
    \label{fig:femDirichelet}
\end{figure}

Results are shown on Figure~\ref{fig:femDirichelet}. Solving the problem took approximately 3 seconds. Stress and strain tensors have been computed. {\color{red}An amazingly nice discussion will be here}.
